First Flight Performance of the Micro-X Microcalorimeter X-Ray Sounding Rocket

The flight of the Micro-X sounding rocket on July 22, 2018 marked the first operation of Transition-Edge Sensors and their SQUID readouts in space. The instrument combines the microcalorimeter array with an imaging mirror to take high-resolution spectra from extended X-ray sources. The first flight target was the Cassiopeia~A Supernova Remnant. While a rocket pointing malfunction led to no time on-target, data from the flight was used to evaluate the performance of the instrument and demonstrate the flight viability of the payload. The instrument successfully achieved a stable cryogenic environment, executed all flight operations, and observed X-rays from the on-board calibration source. The flight environment did not significantly affect the performance of the detectors compared to ground operation. The flight provided an invaluable test of the impact of external magnetic fields and the instrument configuration on detector performance. This flight provides a milestone in the flight readiness of these detector and readout technologies, both of which have been selected for future X-ray observatories.

==> sections/ACSImpact.tex <==

%\subsubsection{Impact of ACS Failure}
%\label{sec:flight_magnetic_field}


% \begin{figure}
% 	\begin{center}
% 		\includegraphics[width=.48\textwidth]{figs/RADec_time.png}
% 		\includegraphics[width=.48\textwidth]{figs/RADec_time_polar.png}
% 	\end{center}
% 	\caption{Plot of right ascension (RA) vs. declination (Dec) of the instrument optics. The colorbar shows the time during flight and the data shown is from 111~s to 431~s, which is slightly longer than the science observation window.\rcom{Placeholder graph for now. Need to decide which one and put Cas-A: RA 350.85 DEC: 58.815. need to be careful on path line thickness, here looks like we get close but Cliff's it does not. On polar plot, change radius units.}}
% 	\label{fig:RADec_time}
% \end{figure}

%\begin{figure}
%	\begin{center}
%		\includegraphics[width=\textwidth]{figs/36245-xrays_16x8.pdf}
%	\end{center}
%	\caption{\acom{Appropriate for a thesis, not relevant for this paper, asking people to read in too much into the sources} Plot of right ascension (RA) vs. declination (Dec) pointing direction of the the Micro-X payload during flight. The plot consists of dots of reconstructed payload orientation from different subsystems during the flight. Light orange are gyroscope solutions from the from the Celestial Attitude Control System (CACS) from launch to 50 sec, dark orange are gyroscope solutions from the from the S19 Aerodynamic Guidance System from 62--440 sec, and blue (mostly under the orange dots) are CACS solutions from 88--440 sec. Green points correspond to pointing solutions from the on-board star tracker video and the star field at the time. Blue and red crosses indicate the location of X-ray sources from the ROSAT All-Sky Survey Bright Source Catalogue with flux rates of above 1 and 10 counts per second, respectively. The red star symbol indicates the location of the intended target (CAS-A) at RA 350.85, DEC: 58.815. The closest approach to the target was approximately 7.5 degrees at around 350 seconds into flight. Regions above the dotted purple line were above the visible horizon during the flight.}
%	\label{fig:RADec_time}
%\end{figure}


%\rcom{This section should include baseline/magnetometer graphs and statements. Renee and Tali to get together and wrap up the timing issue with baseline data, discrepancy between mag x and mag y. RA/DEC polar plot with Cas-A marked. Dan's event timestamp plot, Helmholtz testing, Pulse height and decay times versus direction of magnetic field - basically the old subsection called "TES response" }



==> sections/SNR_science.tex <==
% !TEX root = ../instrument_paper_revB.tex

%%PUT ANY OF THIS IN INTRO???%%
%Much of the detailed physics of astronomical sources is accessible only through plasma %kinematic, temperature, ionization, density and abundance
%diagnostics that require moderate to high resolution spectroscopy ($E/dE = R \gg 20$).  High resolution spectra have long been available at optical and radio wavelengths. For point sources, the Chandra and XMM-Newton grating spectrometers have demonstrated the power of $R \gg 20$ spectroscopy in X-rays~\citep{Paerels:2003}. Results range from measuring precise chemical abundances in stellar coronae~\citep{Gudel:2004} to solidifying the cooling flow mystery in clusters of galaxies~\citep{Peterson:2003} and uncovering massive outflowing winds in active galaxies~\citep{Crenshaw:2003}.  The dispersive nature of the high resolution spectrometers on Chandra and XMM-Newton have sharply limited their use for sources with any significant angular extent; the XMM RGS spectra are an improvement over moderate resolution CCD spectrometers only if a source is more compact than 3$'$. Thus, virtually all of the brightest extended sources in the sky are currently inaccessible for detailed study at the highest spectral resolution. In addition, dark matter searches which look for an X-ray line from the decay or annihilation of dark matter in the Milky Way are optimized with large grasp observations, as are studies of the soft X-ray background. This type of observation is not possible with current observatories. These gaps will be filled by Micro-X. The tremendous scientific potential of high-resolution spectroscopy is surveyed in~\citep{Paerels:2003,Paerels:2010,AthenaIFU:2016}. 

%*** Keep this if you have space!
% For
%all these sources, we will examine the line structures to ascertain
%the dynamic properties of the emitting gas, and perform plasma line
%diagnostics to infer the physical conditions of the X-ray emitting
%plasma.  For the Puppis A ejecta knot, we will look for velocity
%structures that give clues to the dynamical state of a variety of
%ejecta elements, ranging from O and Ne synthesized by the progenitor,
%to Si that was synthesized during the supernova explosion.  In the
%case of M87, we will search for the kinematic signature of the heating
%of the X-ray emitting gas that must be taking
%place~\citep{Forman:2005}.  For Cas A, we will capitalize on
%improvements in the mirror later in the mission to examine the
%velocity structure of compact ejecta knots on 30$''$ angular
%scales. 
%For all the sources, plasma line diagnostics will provide insights into the temperature and (in the case of the SNRs) ionization structure of the gas, as well as enabling more precise estimates of the element abundances.  
%For SNRs, Micro-X will enable better understanding of the nature of the progenitors and their explosions. %For M87, we will shed light on the chemical enrichment of the gas and the absence of a central cooling flow at temperatures below 0.6 keV. 
%%%%%%%%%%%%%%%%%%%%%
%The point: we know it's core-collapse even if most X-ray is not ejecta
Puppis~A exploded in a supernova around 4000~years ago~\citep{Becker:2012, Zavlin:1999}. The resulting middle-aged SNR located at $\sim$2.2~kpc~\citep{Reynoso:2003}, is one of the brightest in the soft X-ray band. Its diameter is estimated to be roughly 30 pc. As most of the X-ray emission from Puppis~A exhibits the sub-solar elemental abundances indicative of shock-heated ambient gas, it is believed to arise from the interaction of the remnant shock with its complex environment rather than coming from SNR ejecta~\citep{Dubner:2013, Luna:2016}. Enough ejecta emission has, however, been observed at both optical~\citep{Winkler:1985a,Winkler:1988} and X-ray wavelengths~\citep{Canizares:1981, Flanagan:1990, Tamura:1994, Hwang:2008, Katsuda:2008, Katsuda:2010,Katsuda:2013} to firmly classify Puppis~A as the remnant of a core-collapse explosion. This designation is further confirmed by the properties of an X-ray emitting neutron star believed to have been produced by the Puppis~A supernova~\citep{Petre:1996a, Winkler:2007a, Gotthelf:2009a}. 

%The point: big and bright enough for Micro-X specs
Within this large remnant, ejecta concentrations (``knots'') are particularly interesting to observe in the X-ray regime. %The first motion of the O-rich ejecta were confirmed when~\cite{Katsuda:2008} used XMM-Newton EPIC X-ray data to demonstrate that one of the O ejecta knots is significantly blueshifted.~\cite{Katsuda:2013} constrained the blueshift velocity to be $\sim$1500~km/s using XMM-Newton RGS data. 
The primary Micro-X target is the BEK, shown in Figure~\ref{fig:moneyplot} (left), which is the interaction site of the SNR with a dense ambient cloud~\cite{Hwang:2005}. It is one of the brightest features in Puppis~A. The elements observed in the BEK by Chandra and XMM-Newton --- O, Ne, Mg, Si, and Fe --- have strong lines that can be well resolved by Micro-X, as shown in Figure~\ref{fig:moneyplot} (right), and the main morphological features are well-matched to the Point Spread Function (PSF) of the Micro-X optics. The BEK is bright enough to be compatible with a 300~s sounding rocket flight; a simulation based on the Chandra spectrum of the BEK, shown in Figure~\ref{fig:moneyplot} (right), projects $\sim$17,000 counts in a single Micro-X observation. 

%Point: what is CX, why look here
The primary science goals of the Micro-X BEK observation are to understand the importance of charge exchange (CX) reactions and to study particle acceleration at the shock front.~\cite{Lallement:2004} showed that CX X-ray emission strength can be comparable with thermal emission in thin layers at the edge of a SNR. The CX contribution is more important where the local density is higher, motivating the search for CX emission from the BEK. The analysis of the BEK from XMM-Newton RGS data~\cite{Katsuda:2012} found an enhanced ratio of the O forbidden to resonance lines. This cannot be explained by a normal collisional plasma, and the conclusion is that CX processes, which originate from interactions between highly ionized atoms and neutrals, contribute significantly to the X-ray emission from the BEK. However, the spectral response of the RGS for extended sources, including the BEK, is very complex given the instrument response, and this claim of the CX detection remains under debate. The Micro-X instrument is well-suited to this analysis, and this observation could conclusively establish the presence of CX at the BEK. 

\begin{figure}[hbt]
    % \centering
    %\includegraphics[width=0.49\textwidth]{figs/puppis_comp_FoV}
    \includegraphics[height=2.4in]{figs/PuppisAKnotHighRes.png}
    \includegraphics[height=2.4in]{figs/PuppisASpectrum.png}
    \caption{The Micro-X field of view will cover the BEK region of Puppis~A (left), shown over a three-color image of Puppis~A from~\cite{Katsuda:2010}. Red, green, and blue correspond to the 0.5--0.7 keV (mostly O K-shell lines), 0.7--1.2 keV (mostly Ne K-shell lines), and 1.2--5.0 keV bands, respectively. The simulated Micro-X spectrum (right) of the BEK (red), shown with the Chandra spectrum of the BEK (black), can resolve previously indistinguishable emission lines. The inset shows the oxygen He-like triplet (the forbidden, intercombination, and resonance lines~\cite{Porquet:2000}), clearly distinguishable with 4 eV resolution. } 
    \label{fig:moneyplot}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%

%%% THIS WAS REPLACED WITH UNA'S VERSION (ABOVE): The initial Micro-X observation will target the bright, middle-aged galactic SNR Puppis A.  This remnant was identified as the product of a core-collapse explosion on the basis of fast-moving optical knots highly enriched in O~\citep{Winkler:1985a}.  The subsequent discovery of a neutron star associated with the remnant~\citep{Petre:1996a}, measurement of its high-velocity proper motion~\citep{Winkler:2007a}, and the measurement of its rotation period~\citep{Gotthelf:2009a} confirm the core-collapse origin of Puppis A and add to its interest.  %Thirty five years ago, Puppis A was the target of one of the earliest successful high-resolution X-ray spectral observations with the Einstein Focal Plane Crystal Spectrometer~\citep{Flanagan:1990, Canizares:1981,Winkler:1981}. The observations were of limited energy range and sensitivity, and the spectra obtained were integrated over the $3' \times 30'$ aperture size. Even so, these observations showed that Puppis~A is a bright source of X-ray emission lines of O and Ne.
%%%%THIS WAS REPLACED WITH UNA'S PARAGRAPHS ABOVE: Most of the optical knots are located in the northeastern portion~\citep{Winkler:1988}, whereas the stellar remnant is moving in the opposite direction (southwest)~\citep{Petre:1996a, Becker:2012}. Notably, this is consistent with some theoretical predictions; a stellar remnant is kicked away by the SN ejecta expelled preferentially in one direction~\citep{Wongwathanarat:2013}. Therefore, Puppis A is an extremely important object to study the mechanism of core-collapse SN explosions. 


%As a middle-aged remnant, Puppis A straddles the division between young objects whose X-ray emissions are dominated by their supernova debris, or ejecta, and older remnants that have lost all trace of their ejecta.  
%In spite of its estimated age of 4000 years, Puppis A is one of only a handful of remnants that shows fast-moving ejecta in optical emission. <- commented out by HY. I think we should focus on X-ray observations in this chapter


% Puppis A is one of the brightest SNRs in the soft X-ray band (and thus suitable as a target for Micro-X), showing evidence for X-ray emitting ejecta, with even the earliest Einstein observations suggesting an overall O abundance enhancement~\citep{Flanagan:1990,Canizares:1981}. The CCDs on the ASCA X-ray Observatory showed that Ne is particularly enhanced in the fainter western and southern regions of the remnant~\citep{Tamura:1994}, and Chandra observations near a complex of shocked interstellar clouds known as the Bright Eastern Knot (BEK) also showed regions of localized abundance enhancement~\citep{Hwang:2005}.
% The first motion of the O-rich ejecta were confirmed via Doppler shift of X-ray emission lines as well. Using XMM-Newton EPIC,~\cite{Katsuda:2008} revealed that one of the O ejecta knots is significantly blueshifted. More recently,~\cite{Katsuda:2013} constrained the blueshift velocity to be $\sim$1500~km/s using XMM-Newton RGS. 

% The RGS observation was applied to the BEK as well~\cite{Katsuda:2012}. They discovered enhanced ratio of the O forbidden to resonance lines, which cannot be explained by a normal collisional plasma. Therefore, they concluded that the charge exchange (CX) processes, which originates from interactions between highly ionized atoms and neutrals, contribute significantly to the X-ray emission from the BEK. 
% %The CX can take place if an SNR is interacting with dense surrounding clouds, as it originates from interactions between highly ionized atoms and neutrals~\citep{Serlemitsos:1973}. 
% Reference~\cite{Lallement:2004} theoretically showed that CX X-ray emission can be comparable with thermal emission in thin layers at the SNR edge. Since the CX contribution becomes more important when the ambient medium density is high, it might be reasonable that this emission was detected from the BEK where the SNR shock is interacting with the dense cloud~\citep{Hwang:2005}. However, the spectral response of the RGS for extended sources, such as the Pup A BEK, %is too complicated, 
% is very complex, so the claim of the CX detection is still under debate. Therefore, our proposed Micro-X observation, with much better energy resolution and response, is crucial to conclusively establish the presence of CX at the BEK. 

%{\it Another SNR from which detection of CX is claimed is 1E0102.2--7219 (Rasmussen et al.\ 2001), but this was not confirmed by Chandra grating observations (Flanagan et al.\ 2004).} \com{Use it if you find a good place to insert. Otherwise, just delete it.}



 %Although subsequent observations combined with advances in plasma modeling have not confirmed the quantitative magnitude of the ejecta enhancement inferred by the FPCS, they have clearly confirmed the presence of X-ray emitting ejecta in the remnant. 
%%%%%%%%%%%%%Repeat from 1st image
% \begin{wrapfigure}{r}{4in}
% \begin{center}
% \vspace{-12pt}
% \includegraphics[width=4in]{figs/full.pdf}
% \end{center}
% \caption{Mosaic of observations of the Puppis A supernova remnant as imaged by the {\it XMM-Newton} and {\it Chandra} X-ray telescopes. The boxes are the 11.8$'$ Micro-X fields of view overlaid on the positions of the Si ejecta knot and the bright eastern knot (BEK).  \textbf{Inset left:} {\it Chandra} ACIS image of the BEK, where the complex structure of the knot is apparent. \textbf{Inset right:} Equivalent width (EQW) image of the Si blend near 1.86 keV from the Suzaku Observatory that delineates the ejecta knot~\citep{Hwang:2008a}. }\label{fig:PupA-xray}
% \vspace{6pt}
% \end{wrapfigure}


%O and Ne ejecta are the unmistakable signature of massive progenitors that synthesize these elements hydrostatically during their lifetimes before the supernova explosion, while much of the Si ejecta was synthesized explosively during the supernova itself. The abundance profile of all the elements
%in the ejecta help to constrain the properties of the supernova progenitor, but it is the explosively synthesized ejecta such as Si and Fe deep in the core of the exploding star that have the greatest potential to shed light on the supernova explosion itself. This makes the identification of Si-emitting ejecta particularly interesting.



%The improved sensitivity and spectral resolution of the CCDs on the Suzaku X-ray Observatory have led to the identification of a coherent, large-scale ejecta feature in ``equivalent width'', or line/continuum images, of Si emission in Puppis~A~\citep{Hwang:2008a}, Figure~\ref{fig:PupA-xray}(right inset).  This roughly 8$'\times10'$ region is located in the north/northeast region of the remnant, somewhat farther out in radius than the optically-identified O ejecta.  
%Much of the imprint of the supernova explosion that formed Puppis~A has been lost in the intervening 4000 years, %--the more so, given the extremely complicated environment into which the remnant is evolving--
%but the fragments of debris originating from deep within the star still hold valuable clues to understand the explosion.  %Despite its relatively advanced age, Puppis~A remains one of the very few remnants of definitively known core-collapse explosions that reveal this deep-lying Si ejecta.





%The high velocities of the optically emitting ejecta (1500 km/s) and the high velocity recoil of the neutron star (also $\sim$1500 km/s) suggest that X-ray emitting ejecta should also have high velocities.  Indeed, XMM-Newton observations of a small region corresponding to a bright optical ejecta feature known as the $\Omega$ knot (located at the southeastern edge of our target Si ejecta knot within our FOV~\citep{Katsuda:2008a}) show evidence for blueshifted emission lines corresponding to velocities of 1500-3000~km/s.  They also show evidence for temperature and abundance differences on 1$'$ angular scales.  The Suzaku observations show that the large ejecta knot can be subdivided into two parts, with the northern half dominated more strongly by Mg and Si than the southern half, in which the O and Ne emission are relatively stronger.  The element abundance maps obtained by Suzaku confirm that this entire feature is enhanced not only in Si, but also in O, Ne, Mg, and possibly Fe.

%All of the ejecta elements observed by Suzaku and XMM-Newton--O, Ne, Mg, Si, and Fe--have strong lines that will be accessible to Micro-X.
%In fact, the CCD spectra of Puppis A fall off rapidly at energies
%above 3 keV, making it a natural match to the Micro-X bandpass.  And
%While Chandra observations of the region do show that there is some structure on smaller angular scales, this $8'\times10'$ feature is overall well-matched to the modest angular resolution of the initial Micro-X mirror and its field of view.  A simulation based on the spectrum observed by Suzaku for the entire knot yields about 17,000 counts in a 300~s Micro-X observation (Figure~\ref{fig:moneyplot}).


%***Organize in bullets if space permits:
%The goals of our Micro-X observation of the Si ejecta knot in Puppis A are to:
%\begin{itemize}\vspace{-6pt}
%\item Search for velocity shifts in the various emission lines and measure the line structures to obtain information about the dynamics of the
%various ejecta elements.  \vspace{-6pt}
%\item Perform plasma diagnostics for the various emission lines of individual elements to ascertain how similar or different the
%thermodynamic states of the various elements are.\vspace{-6pt}
%\item Refine estimates of element abundances in the ejecta. \vspace{-6pt}
%\end{itemize}

%Velocity and dynamics will give us direct information as to how well-mixed the ejecta are, and in particular, whether there were any differences in the dynamics of the outlying O and Ne ejecta compared to the inner Si and Fe ejecta.  Although velocity shift measurements have been attempted with CCD spectra~\cite{Katsuda:2008a}, those moderate resolution spectra do not resolve individual lines so that the energy shift of any particular line is partly obscured by the
%presence or absence of weak lines in the blend.  This is especially true for supernova remnant plasmas, for which the ionization state of the gas is still evolving toward equilibrium.   

%At the next level, we will study the thermodynamics of the plasma.  The progress to ionization equilibrium depends on both the density of the gas and the
%shock time, so that the ionization age serves as an important indicator of the evolution of the remnant.  Complexities in the temperature structure are also expected, as a range of temperatures is indicated in Chandra, XMM-Newton, and Suzaku observations.  In the case of the Fe~L lines, the mere identification of the L lines present in the spectrum gives a diagnostic of the range of temperatures in the gas.  

%Finally, once the dynamic effects and the physical properties of the emitting gas are understood, the high resolution Micro-X spectrum will provide the means to refine estimates of element abundances in the ejecta. The detailed insights into the temperature and ionization structure are crucial to such an effort.  Although the ejecta knot is only a relatively small part of the total ejected material, its large physical scale suggests that it may be a fair representation of the whole. The Micro-X observation would then enable a detailed comparison to the nucleosynthesis predicted in core-collapse SN models. 

%Figure~\ref{fig:moneyplot}(bottom) shows a simulation of the Micro-X spectrum for \uxf{1}. Many individual lines from different elements are visible. The inset shows the oxygen He-like triplet, with a 1500~km/s blueshifted version in dashed blue, showing the power of Micro-X to both measure the triplet component fluxes and accurately measure line velocities.

%\com{Daniel, CR acceleration text starts here. We are doing better on page length so you don't need to cut this down, although I think it would be better if it were a bit shorter :)}


%Daniel's text:
%\acom{AH: I tried to re-write, but I do no understand what is being said. Some Q's to make clear: what do the younger SNRs have to do with Puppis? Is the issue that the gamma signal in Puppis should have a corresponding X ray signal but it doesn't? Or that Puppis is different from others? What do IC443/W44 mean for Puppis? I think there are links that it is assumed I know to make, but I don't know what they are... }

%Daniel's text (old version):
The connection between SNRs and cosmic ray (CR) acceleration is one of the fundamental outstanding questions in SNR science. $\gamma$-rays are the primary observation channel for CR acceleration in SNRs, and X-ray observations of CX in SNRs constrain $\gamma$-ray emission models in the SNR.   
CR hadrons are projected to carry away a significant fraction of the supernova explosion energy and distribute it across the Galaxy. However, hadronic CR production has not yet been clearly shown to occur in SNRs, and the acceleration process itself is not well understood. The hadron-proton collisions from CRs interacting with regions of high-density material produce neutral pions that decay and emit $\upgamma$-rays~\cite{Claussen:1997}. Since CR leptons can also produce $\upgamma$-rays through bremsstrahlung or inverse Compton emission, isolating the origin of the $\upgamma$-ray emission in SNRs has generally proved to be difficult. However, the $\upgamma$-ray emission from SNRs such as IC443 and W44, which are interacting with dense clouds of material has been shown to predominantly originate from pion decay~\citep{Ackermann:2013}. 

The eastern side of Puppis~A is also interacting with dense clouds of material, and MeV-GeV observations with Fermi-LAT reveal significant $\upgamma$-ray emission in the eastern side of Puppis~A ~\citep{Hewitt:2012,Xin:2017}.
The emission line information from Micro-X will determine how significant CX emission is in this region. Since the ratio of CX to thermal emission depends on the cloud density, the relative velocity between neutrals and ions, and the electron density of the hot plasma, the Micro-X observation will contribute to the exploration of whether the $\gamma$-ray spectrum can be explained with re-acceleration, especially regarding the $\gamma$-ray spectral break that may be introduced by CR propagation dampening by neutrals.

%This paragraph was nixed by Tali to try to lower the CR acceleration pedagogy in the paper:
%The spectrum of this $\upgamma$-ray emission shows a significant break at approximately 8 GeV. The shock velocities in W44, IC443, and the BEK in Puppis A are projected to be too low for efficient acceleration of CR particles. However, in evolved SNRs interacting with dense material, re-acceleration of the ambient CR population can boost the relativistic particle population considerably. With subsequent compression in radiative shocks, where the compression ratio is very high, this process may be sufficient to explain the bright radio emission~\citep{Vanderlaan:1962,Blandford:1982} and $\upgamma$-ray emission~\citep{Uchiyama:2010,Lee:2015} from such SNRs. The re-acceleration process flattens the ambient CR spectrum for both electrons and protons. The effects of ion-neutral damping of Alfven waves in the partially neutral upstream medium introduces a break in the particle spectra, with a steepening by one power in momentum above the break~\citep{Malkov:2011}. This is consistent with what is observed from $\gamma$-ray observations of SNRs interacting with molecular clouds, like W44~\citep{Lee:2015}. The position of the break is dependent upon the upstream neutral fraction which, in turn, depends on several factors, such as the speed of the shock (which produces the ionizing photons).  

 


%Daniel's text (old version):

%One of the key outstanding issues in SNR science is the connection between these objects and cosmic ray (CR) acceleration. CR hadrons are believed to carry away a significant fraction of the explosion energy and distribute it across the Galaxy, yet we lack clear evidence of their production in SNRs, and a detailed understanding of the acceleration process and its effects on the SNR plasma. In contrast to several younger SNRs, the X-ray spectrum of Puppis A shows no evidence of non-thermal emission. In these younger SNRs, CR electrons are accelerated to TeV energies, interacting with the locally compressed and amplified magnetic field (e.g.,~\cite{Koyama:1997}. However, Fermi-LAT observations reveal significant gamma-ray ($\gamma$-ray) emission in the eastern side of Puppis~A~\citep{Hewitt:2012,Xin:2017}, indicating an enhanced CR particle density. The spectrum of this $\gamma$-ray emission shows a significant break at approximately 8 GeV. The emission line information from Micro-X will determine how significant CX emission is in this region. Since the ratio of CX to thermal emission depends on the cloud density, the relative velocity between neutrals and ions, and the electron density of the hot plasma, the Micro-X observation will contribute to the exploration of whether the $\gamma$-ray spectrum can be explained with re-acceleration, especially regarding the $\gamma$-ray spectral break that may be introduced by CR propagation dampening by neutrals. 

%The proton-proton interactions from CRs hitting regions of high-density material produce neutral pions that decay and emit $\gamma$-rays~\citep{Claussen:1997}. The $\gamma$-ray emission from SNRs IC443 and W44, both interacting with dense molecular clouds, has been shown through analysis of Fermi-LAT data to be predominantly hadronic in origin~\citep{Ackermann:2013}. The shock velocities in W44, IC443, and the BEK in Puppis A, are all thought to be too low for efficient acceleration of CR particles. However, in evolved SNRs interacting with dense material, re-acceleration of the ambient CR population can boost the relativistic particle population considerably. With subsequent compression in radiative shocks, where the compression ratio is very high, this process may be sufficient to explain the bright radio emission~\citep{Vanderlaan:1962,Blandford:1982} and $\gamma$-ray emission~\citep{Uchiyama:2010,Lee:2015} from such SNRs. The re-acceleration process flattens the ambient CR spectrum for both electrons and protons, and the effects of ion-neutral damping of Alfven waves in the partially neutral upstream medium introduces a break in the particle spectra, with a steepening by one power in momentum above the break~\citep{Malkov:2010}, consistent with what is observed from $\gamma$-ray observations of SNRs interacting with molecular clouds, like W44~\citep{Lee:2015}. The position of the break is dependent upon the upstream neutral fraction which, in turn, depends on several factors, such as the speed of the shock (which produces the ionizing photons).  

%The Micro-X observation of the BEK will study the physics of a shock front interacting with very dense clouds of material. %, expanding on the detailed work presented in~\citet{Hwang:2005}. 
%A {\it Chandra} ACIS observation %(see the left inset in Figure~\ref{fig:PupA-xray}) 
%allowed for a spatially resolved spectral study of the BEK~\citep{Hwang:2005}. Using CCD-spectra, maps of temperature and abundance ratios of O and Ne were constructed to illustrate variations in the nature and conditions of the shocked material in this area. Additionally, the high-spatial resolution of {\it Chandra} revealed substructures in the shock-heated gas, which are somewhat similar to those observed in laboratory laser experiments designed to model such conditions~\citep{Hwang:2005,Klein2003}.  Hence, this study identified cloud-shock interaction in a relatively mature stage of evolution. 

%If the BEK is the source of the $\gamma$-rays, this will be the first high energy resolution X-ray characterization of a CR acceleration/re-acceleration site in an SNR. Micro-X will provide new tools to characterize the properties of shocks, such as their velocity, and those of the plasma, including its density profile and post-shock temperature. %\com{Detailed projections for this observation are found in X.} 

% ended here

%In addition, the particle acceleration process at the shocks of SNRs is expected to modify the hydrodynamic evolution of the object and the properties of its thermal X-ray emission (e.g.,~\citep{Castro2011}). Micro-X will provide new tools to characterize the properties of shocks, such as their velocity, and those of the plasma, including its density profile and post-shock temperature, through the study of thermal X-ray emission. %In turn, this will allow us to gain a much deeper understanding of the mechanism of cosmic ray production, evidenced by the $\gamma$-ray emission detected in the direction of the remnant, and how it couples to the properties of the surrounding material and the shock.
% Cosmic rays interacting with regions of high-density material are expected to result in $\gamma$-ray emission from the decay of pions generated by proton-proton interactions. Hence, studying a region of an SNR that appears to be propagating into a molecular or atomic cloud complex is particularly important when searching for signatures of CR acceleration, and in particular, clear signals of hadronic emission. 
%\begin{wrapfigure}{r}{4in}
%\vspace{-24pt}
%\begin{center}
%\includegraphics[width=4in]{full.pdf}
%%\includegraphics[width=0.49\columnwidth]{spitzer.pdf}
%\end{center}
%\vspace{-12pt}
%\caption{}
%\label{fig:PupA-xray}
%\vspace{-12pt}
%\end{wrapfigure}
%

%Non-thermal X-ray emission from young shell-type SNRs, such as RX J1713.7-3946~\citep{Koyama1997}, and Vela Jr.~\citep{Aschenbach1998}, is believed to be the result of synchrotron radiation from electrons accelerated to TeV energies at the SNR shock through diffusive shock acceleration (DSA). Observations of TeV $\gamma$-ray emission from some SNRs also support the scenario where particles are being accelerated to energies approaching 10$^{15}$ eV in these objects~\citep{Enomoto2002,Katagiri2005}. However, broadband observations and modeling are required to establish the origin of these high energy photons, since the characteristics of the $\gamma$-ray emission alone are not sufficient to clearly establish if these originate from leptonic emission mechanisms (such as inverse Compton or non-thermal bremsstrahlung emission), or from relativistic hadrons interacting with the ambient medium. 

% The characteristics of the thermal X-ray emission from SNRs detected in $\gamma$-rays have been used successfully to gain insight into the cosmic ray acceleration process. %Studies of the hydrodynamic evolution and the properties of the shocked medium and ejecta have yielded important information about CR production. %The X-ray morphology of Tycho's SNR and SN~1006 indicates that the shock compression ratios in these objects have been modified by the acceleration of cosmic ray ions~\citep{Warren2005,Cassam2008}, while comparisons of the postshock plasma temperatures and shock velocities observed in SNRs 1E~0102.2-7219 and RCW~86 also point to a significant fraction of their explosion energy being placed in relativistic particles~\citep{Hughes2000,Helder2009}.  
% Hydrodynamic simulations of SNRs which include  particle acceleration at the shock self-consistently, and calculate and track the non-equilibrium state of the post-shock plasma through the evolution of the system, have used thermal X-ray emission as a key diagnostic in understanding the observed broadband properties of some remnants.~\citet{Castro2012} used such modeling and X-ray line emission observed with the {\it XMM-Newton} EPIC cameras to conclude that the $\gamma$-ray emission detected with the {\it Fermi} Large Area Telescope (LAT) in the direction of SNR CTB~109 is the result of a combination of emission from accelerated leptons and hadrons.~\citet{Ellison2010} instead used the lack of line emission observed in RX J1713.7-3946 as a constraint in their modeling, which suggests that its $\gamma$-ray emission is dominated by inverse Compton radiation.

%The bright eastern knot (BEK) in the SNR Puppis A represents an excellent laboratory for the study of the interaction between SNRs and dense clouds of gas. Cosmic rays interacting with regions of high-density material are expected to result in $\gamma$-ray emission from the decay of pions generated by proton-proton interactions. Hence, studying a region of an SNR that appears to be propagating into a molecular or atomic cloud complex is particularly important when searching for signatures of CR acceleration, and in particular, clear signals of hadronic emission. While TeV and GeV observations have revealed $\gamma$-ray emission from several SNR-molecular cloud systems (e.g.,~\citet{Aharonian2006,Abdo2009,Castro2010}), X-ray emission from these objects is characterized by a centrally peaked morphology. Recently, observations with the {\it Fermi}-LAT revealed an unresolved $\gamma$-ray source, with detection significance $>14\sigma$, with emission centered on the eastern part of the Puppis A remnant. While the study of this region is ongoing, recent preliminary work by our team suggests these $\gamma$-rays originate from cosmic ray hadrons accelerated at the shock which are interacting with extremely dense material with which the shock is interacting. 

%\noindent$\bullet$ Talk about SNR/MC interactions, and connection with gamma rays. Mention Fermi detection.
%\noindent$\bullet$ Talk about Hwang 2005 and the nature of the BEK in X-rays.




%The objectives of the Micro-X observation of the BEK are: (1) use line broadening and ratios to obtain information about the dynamics of elements in different regions of the shocked high-density cloud complex; and (2), use plasma diagnostics for the various emission lines of each element to establish variations in the thermodynamic conditions of different elements across the interaction region. Meeting these goals, we will be able to characterize the interaction region between an SNR and a high-density cloud complex with spatially resolved high-resolution X-ray spectra for the first time, and gain crucial insight into the nature of such systems, obtaining a very clear picture of the conditions in a region where cosmic ray acceleration is known to be taking place.


%The goals of the Micro-X observation of the Si ejecta knot in Puppis A
%are multi-faceted.  At the most straightforward level, we will
%search for velocity shifts in the various emission lines and measure
%the line structures to obtain information about the dynamics of the
%various ejecta elements.  Such observations will give us direct
%information as to how well-mixed the ejecta are, and in particular,
%whether there were any differences in the dynamics of the outlying O
%and Ne ejecta compared to the inner Si and Fe ejecta.  Although
%velocity shift measurements have been attempted with CCD spectra~\cite{Katsuda:2008a},
%those moderate resolution spectra do not resolve individual lines so
%that the energy shift of any particular line is partly obscured by the
%presence or absence of weak lines in the blend.  This is especially
%true for supernova remnant plasmas, for which the ionization state of
%the gas is still evolving toward equilibrium.  At the next level, we
%will perform plasma diagnostics for the various emission lines of
%individual elements to ascertain how similar or different the
%thermodynamic states of the various elements are. The progress to
%ionization equilibrium depends on both the density of the gas and the
%shock time, so that the ionization age serves as an important
%indicator of the evolution of the remnant.  Complexities in the
%temperature structure are also expected, as a range of temperatures is
%indicated in Chandra, XMM-Newton, and Suzaku observations.  In the
%case of the Fe L lines, the mere identification of the L lines present
%in the spectrum gives a diagnostic of the range of temperatures in the
%gas.  Finally, once the dynamical effects and the physical properties
%of the emitting gas are understood, a high resolution spectrum, as
%will be provided by Micro-X, will provide the means to refine
%estimates of element abundances in the ejecta.  The detailed insights
%into the temperature and ionization structure are crucial to such an
%effort.  Although the ejecta knot is only a relatively small part
%of the total ejected material, its large physical scale suggests that it may be a
%fair representation of the whole. The Micro-X observation would then
%enable the most detailed comparison to nucleosynthesis models for this
%remnant because it would involve a significant mass of a range of
%elements.

%%%%%%% CAS A %%%%%%%%
%\begin{wrapfigure}{r}{0.4\textwidth}
%	\includegraphics[width=0.4\textwidth]{figs/cas_spec.png}
%	\caption{Cas~A Chandra observation with the simulated high resolution Micro-X spectrum.} 
%	\label{CasSpec}
%\end{wrapfigure}
%The secondary SNR target is Cassiopeia~A (Cas~A), which exploded in a Type IIb core-collapse supernova $\sim$340~years ago \com{cite}. The resulting Supernova Remnant (SNR) is an attractive target because it is very bright, its distance is well-constrained at 3.4~kpc, and it is the second youngest known SNR in our galaxy. Micro-X will observe emission from multiple knots and determine each of their Doppler-shifted velocities. The brightest region in Cas~A is the 200" ``Bright Ring," where material was ejected outwards in the supernova, then compressed and heated by the reverse shock. Micro-X will analyze the Bright Ring to study the effect of post-shock deceleration and turbulence on X-ray-emitting ejecta. Micro-X's high-resolution detectors can separate previously-entangled emission lines in Cas~A for the first time. Roughly 13,000~counts are expected in a 300~second observation, with 5~counts/s on the hottest pixels (see \S \ref{sec:Detectors}). The resulting simulated spectrum is shown in Figure~\ref{CasSpec}, overlaid with the Cas~A spectrum from Chandra \com{cite}; the identification of individual lines will be newly accessible with the high-resolution Micro-X observation.  

In the case of launching when Puppis~A is not visible to Micro-X, the goals of the secondary target Cas~A  observation are to: 1)~measure line fluxes and map emission lines to estimate elemental abundances, 2)~compare plasma diagnostics between elements, 3)~determine system dynamics from Doppler shifts, 4)~constrain nucleosynthesis models. Detailed projections for this observation can be found in~\cite{Rutherford:2013}. 

==> sections/alignment.tex <==
% !TEX root = ../instrument_paper_revB.tex
\subsection{X-ray Mirror Alignment}
\label{sec:alignment}

\hl{I rewrote and added a table to make things more clear. We should think about what photos we want - they'll be critical for people to understand what we're saying.-AH}

The co-alignment of the X-ray mirror, detector array, and star tracker is a five stage process that requires the use of two reference mirrors, shown in Figure~\ref{OpticalBench}~(right), and two alignment fixtures, shown in Figure~\ref{x}. \hl{Add image of stage 1 and stage 2; maybe of whole system installed.} The procedure is designed to keep the vacuum space of the cryostat from being exposed to the external atmosphere. The five steps are laid out in detail below and summarized in Table~\ref{table:alignment}. After flight, each of these relative alignments are checked in the reverse order. 

(1) \textbf{Aligning the flat reference mirrors:}
Two flat reference mirrors, shown in Figure~\ref{OpticalBench}, are used to align the X-ray mirror and the Star Tracker. Before integrating the optics section into the payload, the reference mirrors are aligned to the optical axis of the X-ray mirror using a 50\micron{} light source, to 10~arcsec precision. The removable reference mirror verifies the alignment of the permanent flat reference mirror to the optical axis of the X-ray mirror. It does not fly; it is bolted to the aft end aperture of the X-ray mirror during testing. The permanent flat reference mirror is used in step 5, to align the mirror to the Star Tracker. Once the two reference mirrors are aligned to the X-ray mirror, the optical assembly is installed onto the rest of the instrument. 

(2) \textbf{Aligning the X-ray mirror to the external alignment fixture:}
The “external alignment fixture” is bolted to the aperture valve to align the X-ray mirror to the center of the cryostat aperture. The external alignment fixture is a flat surface with a central hole ($\varnothing$0.5~mm); this plane sits 283~mm away from the detector array. A camera (whose lens has been glued to focus onto the plane of the external alignment fixture) is placed in the central bore of the mirror. The optical axis of this camera is aligned to the central hole of the external alignment fixture by placing shims at the three mating points between the X-ray mirror and the optical bench. The alignment precision is less than 0.5~arcmin, limited by the thickness of the shims, which range from 0.5-5~mm. After aligning the mirror to the aperture valve, the bumpers that keep the mirror from hitting the rocket skin are installed, and the instrument is turned from vertical to horizontal. The alignment is verified in this new configuration before proceeding.  

(3) \textbf{Aligning the external and internal alignment fixtures:}
The “internal alignment fixture” is installed onto the external alignment fixture, with 229~mm separation between their planes. The internal alignment fixture is installed without its lid, so that light can pass unobstructed through its central hole ($\varnothing$0.5~mm). An LED on the external alignment fixture is turned on and shines through the central holes of both alignment fixtures and onto the alignment camera in the central bore of the X-ray mirror. The internal alignment fixture sits on motorized rails, and it is translated in both lateral directions until the intensity of light on the aligmment camera is maximized, indicating that the central holes of the two alignment fixtures are aligned. 

(4) \textbf{Align the internal alignment fixture and the detector array alignment of the X-ray mirror to the detector array:}
A radioactive $^{55}$Fe source is placed inside the internal alignment fixture, which is then hermetically sealed and pumped down to vacuum. The aperture valve is opened to allow X-rays from the internal alignment fixture to hit the detector array. The array is at 75~mK for the alignment, both so that it can detect X-rays and so that it is in its precise flight location, which shifts with respect to room temperature. When aligned, the TES array sees a 3$\times$3 pixel square illuminated in the center of the array. If misaligned, it sees the star pattern that is cut into the external alignment fixture, providing a measurement of how far off the alignment is from the central hole. Misalignment between the mirror and the detectors can be mitigated by modifying the pointing coordinates of the Star Tracker. 

(5) \textbf{Confirm alignment of the Star Tracker and the X-ray mirror:}
The  Star Tracker  replaces  the  alignment camera in the central bore of the mirror to confirm is alignment with the system. A theodolite is used to measure the relative angle of each reference mirror to the Star Tracker. The alignment between the permanent reference flat mirror and the Star Tracker is used to measure any change in the relative alignment during vibration testing. \hl{What happens if it's off? Shim ST? Restart everything?}

\begin{table}
	\begin{centering}
	\begin{tabular}{lll}
		\hline
		\bf{Stage} & \bf{Step} & \bf{Aligned components} \\
		\hline
		1 & 50~\micron{} light source & X-ray mirror + 2 reference mirrors \\
		2 & Install shims & X-ray mirror + 2 reference mirrors + external alignment fixture\\
		3 & Center LED & X-ray mirror + 2 reference mirrors + 2 alignment fixtures\\
		4 & X-rays on TES array & X-ray mirror + 2 reference mirrors + 2 alignment fixtures + TES array\\
		5 & Theodolite & X-ray mirror + 2 reference mirrors + 2 alignment fixtures + TES array + Star Tracker\\
		\hline
	\end{tabular}
\end{centering}
\caption{The X-ray mirror alignment proceeds in steps, aligning new components at each stage, until the entire system is co-aligned. \hl{Massage phrasing}}
\label{table:alignment}
\end{table}

%(6) \textbf{Aligning  the  cryostat  to  the  skin:}
%A  system  of  4  lasers  and  photosensors  track  the relative  motion  of  the  cryostat  (including  the  array)  to  the  skin  (including  the  bulkhead plate).  Comparison of these measurements before and after vibe will reveal if the cryostat returned to its original position after vibration.  The photosensor data will be transmitted during flight.  A description of this system is provided in the \hl {Design Report document}.
%
%%% Do we include this if we didn't use it?? %%%
%\subsubsection{Laser Positioning Calibration}
%
%The Laser Positioning (LP) calibration system measures the position of the cryostat with respect to the rocket skin. This is designed to understand a misalignment of the optics with respect to the detector array in flight. The system tracks the position of two lasers mounted on the cryostat relative to two photodiodes on the hermetic bulkhead. These 10$\times$10~mm$^2$ photodiodes output a position-dependent voltage to a control box. The control box digitizes this output and sends it to telemetry as an RS422 stream. 

==> sections/dark_matter.tex <==
The Micro-X instrument can be built up in two configurations: an imaging configuration for targets that require spatial resolution (e.g., SNRs), and a large-field of view (FOV) configuration for diffuse signals that do not require spatial resolution (e.g., galactic dark matter). Galactic dark matter surrounds the plane of luminous matter in the Milky Way and should produce an all-sky signal as seen from the solar system. If dark matter participates in X-ray-producing interactions, this signal may be in the X-ray band~\cite{Kev_DM}. A notable example is the keV-scale sterile neutrino, which could decay to an X-ray and an active neutrino, producing an X-ray at half the sterile neutrino mass~\cite{DodelsonWidrow, Andre_2020}. 

Dark matter detection in the X-ray band is particularly compelling because several satellites (\textit{Chandra, XMM-Newton, Suzaku}, and \textit{NuSTAR}) observe an excess at 3.5 keV that may be the product of a dark matter interaction~\cite{keVwhitepaper:2017, Kev_DM, Boyarsky:2019, Bulbul:2014, Boyarsky2018}. This excess is reported from the Galactic Center, galaxies, and galaxy clusters. It may be of atomic origin, but this implies that flux predictions are off by an order of magnitude~\cite{Kev_DM, keVwhitepaper:2017, Boyarsky:2019}; laboratory astrophysics efforts currently point away from an atomic interpretation of this excess~\cite{Shah:2016, Cappelluti:2018, Bulbul:2018, Gall:2019, Hubbard:2021}. Complicating this discussion are the analyses that report no excess, sometimes even using the same data~\cite{keVwhitepaper:2017, Boyarsky:2019}. These analyses are limited by the low signal-to-noise ratio and systematic uncertainties of the instruments~\cite{Dessert_2018, Kev:2020, Boyarsky:2020, Dessert:2020}. The line remains unconfirmed after limited observations with calorimetric resolution as well~\cite{HitomiDM:2017, microxDM:2015}. %They strongly rely on an accurate background model and an understanding of the instrument's systematic errors to return high significance results. 
The nature of this excess requires a new, high-resolution detector to be resolved. 

A sounding rocket mission with high-resolution detectors and a large FOV is well-suited to an indirect galactic dark matter search~\cite{microxDM:2015, HubbardLTD}. Galactic dark matter is an all-sky signal, so a 33$^\circ$ half-angle FOV sounding rocket observes a dark matter flux that is 2700 times that of \textit{XMM-Newton}, making up for its short exposure flight exposure~\cite{microxDM:2015}. Microcalorimeters provide the resolution required to separate the mono-energetic signal from nearby atomic lines~\cite{HitomiDM:2017}. Modifying Micro-X for a large FOV makes it an excellent instrument for this observation~\cite{microxDM:2015, HubbardLTD}. This configuration will remove the X-ray optic. Removing the X-ray optic to widen the FOV and eliminate the decrease in effective area above 2.5~keV due to the optics, as shown in Figure~\ref{fig:optics_eff_area}. Additionally, the aft end apertures will be widened to maximize the FOV, and a new TES array will be used with larger absorbers to increase the detector area. Further details on the dark matter configuration and proposed modifications can be found in~\cite{HubbardLTD}. 

%The expected flux from galactic dark matter depends on the target, the instrument FOV, the integrated column density of the dark matter, and the implied decay rate ($\Gamma$) of the dark matter particle. Previous observations have returned different projections for the expected decay rate. In~\cite{HubbardLTD}, three fluxes (\cite{BoyarskyB:2014};~\cite{Bulbul:2016};~\cite{Boyarsky2018}) are folded into the NFW profile~\citep{NFW} to project the expected flux in the proposed Micro-X flights. 
%
The proposed first target is a region near the Galactic Center that is relatively quiet in the X-ray band. The background spectrum is a nearly flat continuum with 0.6~counts/flight/2.5~eV~\cite{microxDM:2015}. Using the flux derived from~\cite{BoyarskyA:2014}, 20.3$\pm$4.5 signal events are expected in a single flight, corresponding to $>$5$\sigma$ significance~\cite{HubbardLTD}. The projected spectrum of the observation is shown in Figure~\ref{flux_limits} (left). 

\begin{figure}[htb]
\centering
\includegraphics[width=0.35\textwidth]{figs/boyarsky2014_spectrum.png}
\includegraphics[width=0.6\textwidth]{figs/exclusion_north_south.png}
\caption{Simulated Micro-X observation of a quiet region near the Galactic Center (left), focusing on the 3.5 keV region and assuming the dark matter flux from~\cite{BoyarskyA:2014}. The mono-energetic signal (red) is clearly discernible above the background (black), providing a $>$5$\sigma$ result. The background fit is in blue, with the signal fit in green. Projection for additional targets and dark matter fluxes are provided in~\cite{HubbardLTD}. The resulting sensitivity is shown in the parameter space of the sterile neutrino mixing angle $\sin^2 2\theta$ and mass m$_s$. % (which is proportional to the X-ray flux detected) vs sterile neutrino mass (which is twice the X-ray energy) plane. 
The projected exclusion limits for sterile neutrino dark matter are shown for Micro-X North (green dotted) and Micro-X South (red dash-dotted), extending past previous exclusion limits from X-ray observations (shaded) and XQC (black line (\cite{microxDM:2015})). Observations claims from~\cite{BoyarskyB:2014},~\cite{Bulbul:2016}, and~\cite{Boyarsky2018} are shown in red, maroon, and blue dots, respectively}
\label{flux_limits}
\end{figure}

%\begin{wrapfigure}{r}{0.3\textwidth}
%\subfigure{
%\includegraphics[width=0.3\textwidth]{figs/boyarsky2014_spectrum.png}
%\subfigure{
%\includegraphics[width=0.3\linewidth]{south_boyarsky2014.png}}
%\subfigure{
%\includegraphics[width=0.3\linewidth]{figs/combined_boyarsky2014.png}}
%\subfigure{
%\includegraphics[width=0.3\linewidth]{chandra2017_spectrum.png}}
%\subfigure{
%\includegraphics[width=0.3\linewidth]{south_chandra2017.png}}
%\subfigure{
%\includegraphics[width=0.3\linewidth]{figs/combined_chandra2017.png}}
%\subfigure{
%\includegraphics[width=0.3\linewidth]{boyarsky2018_1flight_spectrum.png}}
%\subfigure{
%\includegraphics[width=0.3\linewidth]{south_boyarsky2018.png}}
%\subfigure{
%\includegraphics[width=0.3\linewidth]{figs/combined_boyarsky2018.png}}
%\caption{Micro-X is projected to return world-leading galactic dark matter results with a single flight. The projection of the first target, shown here assuming the dark matter flux from~\cite{BoyarskyA:2014}, returns a $>$5$\sigma$ result. The simulated background data is in black, with the simulated signal in red. The background fit is in blue, with the signal PDF in green. Projection for individual flights and multiple dark matter fluxes are provided in~\cite{HubbardLTD}.}
%\label{spectrum_comparison_plots}
%\end{wrapfigure}
Micro-X will be sensitive to both the reported 3.5~keV excess and to any X-ray signature of dark matter in this energy band. In the case of sterile neutrinos, this sensitivity can be converted into the particle parameters shown in Figure~\ref{flux_limits} (right). The Micro-X observations are statistics-limited, so additional flights will further increase the sensitivity. If a line is detected, Micro-X can discern between dark matter and an atomic origin by mapping the Doppler shift of the line across the Galaxy with multiple flights~\cite{Doppler1, Doppler2}. An atomic background will be co-moving with the Earth, while a dark matter signal will come from the stationary halo. This “velocity spectroscopy” drives the 3~eV resolution specification of the new TES array. 
%A dark matter flux consistent with~\cite{BoyarskyB:2014} or~\cite{Bulbul:2016} would yield an observation of $>$5$\sigma$ significance from Micro-X North or Micro-X South alone (\cite{HubbardLTD}). A dark matter flux consistent with~\cite{Boyarsky2018} would yield a $>$2$\sigma$ observation from Micro-X North and from Micro-X South, and $>$3$\sigma$ from the combined dataset. Even with the most conservative flux estimate, Micro-X will achieve $>$3$\sigma$ sensitivity with the combination of the proposed flights. The Micro-X observations are statistics-limited, so adding additional flights increases the sensitivity even further. The sensitivity of the observation to the specific case of sterile neutrinos is shown in Figure~\ref{flux_limits}, where $m_s$ is the sterile neutrino mass and $\theta$ is the mixing angle between active and sterile states (\cite{GammaRef}). 

%The dark matter decay rate ($\Gamma$) parameter is independent of the exact dark matter particle candidate. In the case of sterile neutrino decays, $\Gamma$ is given by: 
%\begin{equation}
%    \Gamma = \left(1.38 \times 10^{−29} s^{-1}\right) \times \left(\frac{sin^2 2\theta}{10^{-7}}\right) \left(\frac{m_s}{1~keV}\right)^5 \ \ ,
%\end{equation}
%where $m_s$ is the sterile neutrino mass and $\theta$ is the mixing angle between the active and sterile states (\cite{GammaRef}). The sterile neutrino parameters derived from the decay rates and are shown in Figure~\ref{flux_limits} (right). 

%\begin{figure}
%    \centering
%    \includegraphics[width=0.8\linewidth]{exclusion_north_south.png}
%    \caption{Projected exclusion limits for sterile neutrino dark matter from Micro-X North (green dotted) and Micro-X South (red dash-dotted). Previous claims from~\cite{Boyarsky2014},~\cite{Chandra2017}, and~\cite{Boyarsky2018} are shown in red, maroon, and blue dots, respectively. Previous exclusion limits from X-ray observations (shaded) and XQC (black line~\cite{Figueroa2015}) are shown. }
%    \label{exclusion_plot}
%\end{figure}
%
%If a line is detected, it may be from a dark matter interaction or of atomic origin. Micro-X has the ability to discern between these two signals by mapping the Doppler shift of the line across the Galaxy with multiple flights, providing a ``smoking gun" signature of dark matter~\citep{Doppler1, Doppler2}. %This “velocity spectroscopy” requires 0.1\% resolution and drives the 3~eV energy resolution specification of the new array. 
%The Micro-X observation is highly complementary with future XRISM~\citep{XRISM} observations. \mbox{Micro-X} is optimized for the all-sky galactic signal, and its short flight precludes it from observing fainter targets that require a longer exposure with XRISM. XRISM will get excellent spectra from extragalactic sources like galaxy clusters and dwarf spheroidals. Stacking multiple observations throughout the lifetime of XRISM,with a distribution of pointing directions through the Milky Way halo, would require more than 100~Ms of data to accumulate the same signal flux as either Micro-X flight. Thus a combination of data from both experiments is an excellent way to enhance sensitivity to dark matter signals in the X-ray band.  




==> sections/electronics.tex <==
% !TEX root = ../instrument_paper_revB.tex
\subsection{Electrical System}
\label{sec:Electronics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%The Micro-X electrical system includes: 
%\begin{itemize}
%	\item \textbf{Science chain power and readout electronics (\S \ref{sec:Science Chain Electronics})} (two identical sets): The science chain electronics control the operating conditions of the detectors and SQUIDs, and they record data on-board. 
%	\item \textbf{ADR power and control electronics (\S \ref{sec:ADR Electronics})}: The ADR Control (ADRC) electronics use a PID loop to maintain a stable thermal environment at the detector array. 
	%
	%\item \textbf{ADR Position Monitor}: This system includes four sets of laser-photosensor pairs are mounted to the cryostat, the skin, and the vented side of the hermetic bulkhead. The photosensors feed a control box, mounted to the skin, that packages the photosensor information into RS422. The control box takes in 28~V from the power bus and outputs RS422 position information that it sends to telemetry (see \S \ref{ADR Position Monitor}). 
%	\item \textbf{Heat Switch (\S \ref{sec:Valve Electronics})}: This system is only actuated on the ground, and all signals pass from the ground electronics to the science instrument. 
%	\item \textbf{Gate Valve (\S \ref{sec:Valve Electronics}):} The valve, vacuum gauge are mounted to the optics side of the hermetic bulkhead. The motor controller converts commands into motor driver signals. It takes in 28~V power and 5~V timer commands from the telemetry section. It outputs analog housekeeping data to telemetry. 
%	\item \textbf{Pumping Valve (\S \ref{sec:Valve Electronics}):} The motor controller is mounted on the avionics assemby, and the motor and the pressure gauge are mounted to a thermal standoff on the skin. The motor controller converts commands into motor driver signals, and a pressure gauge. It takes in 28~V power and 5~V timer commands from the telemetry section. It outputs analog housekeeping data to telemetry. 
%	\item \textbf{Six vibrometers (\S \ref{sec:NSROC Electricals}):} Two vibrometers are located on the X-ray mirror, two are on the ADR, and two are on the rocket skin. The output from each vibrometer passes through a charge amplifier and an anti-alias filter. 
%	\item \textbf{ST5000 star tracker, shutter door, CDI (\S \ref{sec:NSROC Electricals}):} These are all NSROC systems that have electrical components within the volume of the Micro-X science instrument. Their signals are all routed through the telemetry interface plate. 
%\end{itemize}
%
%Most of the electrical subsystems are physically located in the avionics assembly (Figure~\ref{AvionicsAssembly}), which is an aluminum structure at the forward end of the Micro-X instrument. %Some components of the ADR Position Monitor are mounted to the cryostat, the skin, and the hermetic bulkhead. The gate valve assembly is mounted to the hermetic bulkhead. The vibrometers and charge amplifiers are mounted to the skin, the cryostat vacuum enclosure and the X-ray mirror.

The wiring diagram (Figure~\ref{Wiring}) shows an overview of the instrument's flight electrical system. The dashed line in Figure~\ref{Wiring} marks the interface between the science instrument and the NSROC telemetry (TM) section. The payload has three telemetry (TM) flight downlinks: one 5.0~Mbit/s link for housekeeping data, and two 20~Mbit/s links, one for each science chain. NSROC both records the raw data from the three science instrument telemetry links and transmits it in real time to the scientists. Commands are issued by pre-programmed timers in TM; there is no uplink to command from the ground. Power is supplied by two indepedent, 28~VDC power busses in TM. \com{Add more details or no?}

\begin{figure} [htp]
	\begin{center}
		\includegraphics[width=\textwidth]{figs/updated_wiremap.png}
	\end{center}
	\caption{Science instrument flight wiring overview. \com{Add MPS; rethink layout and what to emphasize visually}} 
	\label{Wiring}
\end{figure}

%The science chain electronics control the operating conditions of the detectors and SQUIDs, while the ADR control electronics control the local environment inside the cryostat. The valve controls allow timer events to actuate, and the laser electronics read in system data and output a data stream. 
%Laser positioning electronics output position data to TM. There are no controls to this system. 
\begin{figure} [htp]
	\begin{center}
		\includegraphics[width=0.8\textwidth]{figs/avionics.png}
	\end{center}
	\caption{Electronics assembly. \com{Relabel; show all in Figure 14}} %\textcolor{red}{Update access panel. "Converter" to "science chain converter". "Magnet" to "ADR magnet"}} 
	\label{AvionicsAssembly}
\end{figure}

\bigskip

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Telemetry Specifications}
%
%The electrical specifications of the instrument and the GSE are provided in the \textit{Electrical Interfaces} document. 
%The payload has three telemetry (TM) flight downlinks: one 5.0~Mbit/s link for housekeeping data, and two 20~Mbit/s links, one for each science chain. 
%
%Commands are issued by pre-programmed timers in TM; there is no uplink to command from the ground. Power is supplied by two indepedent, 28~VDC power busses in TM. 
%
%\begin{adjustbox}{width=\textwidth,totalheight=\textheight,keepaspectratio}
%\begin{table}[htb]
%	\begin{tabular}{|l|l|l|l|}
%		\rowcolor{cyan} Component & Power Bus X (28~VDC) & Power Bus Y (28~VDC) & External (Umbilical)\\
%		\hline
%		Science Chain X & 1.6~A continuous & - & 1.6~A continuous\\
%		\hline
%		Science Chain Y & - & 1.6~A continuous & 1.6~A continuous\\
%		\hline
%		ADR & Redundant: 730~mA continuous & Primary: 730~mA continuous & 2.3~A on rail\\
%		\hline
%		& Stand-by: 50~mA & & Stand-by: 50~mA\\ %\cline{2-2}
%		Gate Valve & Run: 845~mA ($<$60~s) & - & Run: 845~mA ($<$60~s) \\ %\cline{2-2}
%		& Inrush: 1.2~A ($<$ 1~s) & & Inrush: 1.2~A ($<$ 1~s) \\ \cline{2-2}
%		\hline
%		& Stand-by: 43~mA & & Stand-by: 43~mA\\ %\cline{2-2}
%		Pumping Valve & Run: 98~mA ($<$ 60~s) & - & Run: 98~mA ($<$ 60~s)\\ %\cline{2-2}
%		& Inrush: 260~mA ($<$ 1~s) & & Inrush: 260~mA ($<$ 1~s)\\ %\cline{2-2}
%		\hline
%		Heat switch & - & - & 1.5~A\\
%		\hline
%		Laser PM & 150~mA & - & 150~mA\\
%		\hline
%	\end{tabular}
%\end{table}
%\end{adjustbox}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Science Chain Electronics}
\label{sec:Science Chain Electronics}
There are two independent, identical science chains. Each science chain requires 28~VDC and four clock signals from TM. Each science chain includes three enclosures: a converter board enclosure (to convert the 28~VDC to multiple power rails), an interface (IF) board enclosure (for additional amplification of output science signals), and a MUX stack (for SQUID and detector controls and data recording). Each science chain is connected to its own MV encoder \com{[cite- from NM state paper]} in TM that supplies the four digital clock signals. The detectors and SQUIDs are tuned before launch; there is no commanding during flight. 

The MUX stack is the heart of the science chain readout. It holds the Row Address (RA), Quiet DC (QDC),  Digital Feedback (DFB), Regulator (REG) Master Control Board (MCB) cards. The RA card switches the SQ1 bias signals, while the QDC card provides DC biases for the SQ2 amplifier and TES detectors. The DFB card samples the readout and provides digital feedback to the SQUIDs. The REG card supplies regulated power. The MCB controls the other boards, handles the science chain system control, receives and processes both the science data and instrument housekeeping data, handles the on-board storage of the data, and provides the data stream to the telemetry system on the rocket. \com{Has any of this been written up? By NIST? GSFC?}

The full 66~Mbit/s science data stream is written to on-board flash memory, starting at ignition. The full data stream from a subset of pixels is transmitted in real-time, limited by the bandwidth of the TM antennae \com{antenna or encoder limitation?}. This data subset includes the full housekeeping data stream. %For the science data (TM2 and TM3), NSROC provides a bit sync to the instrument and provides the digital data and the bit rate clock to the experimenter GSE. The experimenter team provides the offline frame sync, decommutation and all subsequent data processing and display. 
%The science chain signals are divided into three types: output data, clocks, and commands: \\
%\begin{table} [h]
	%\begin{center}
%	\begin{tabular}{llll}
%		\hline
%		\bf{Signal} & \bf{Data Type } & \bf{Interface} & \bf{Details}\\
%		\hline
%		Bits 0-7 & LVDS & TM; access panel & Science data output\\
%		%Uplink & RS422 & TM; access panel \\
%		Bit rate clock & LVDS & TM; access panel & Encoder-supplied clock\\
%		Read strobe & LVDS & TM; access panel & Encoder-supplied clock\\
%		Major frame & LVDS & TM; access panel & Encoder-supplied clock\\
%		Minor frame & LVDS & TM; access panel & Encoder-supplied clock\\
%		Sequencer Bit command & 0V/5V & TM; access panel & Lanyard command\\
%		SQUID commands & RS422 & Umbilical & GSE command (rail only)\\
%	\end{tabular}
	%\end{center}
%\end{table}
%
%All signals are digital. LVDS signals are 200~mV differential signals with a 1.2~V offset; RS422 signals are 350~mV differential with a 1.17~V offset.  

\com{I am assuming no one cares about the TM matrix. This section can be extremely expanded if desired. }
%\textbf{On the rail:} The signals that are telemetered in flight are sent through a fiber on the rail.  Commands come directly through the umbilical from the experimenter GSE. In addition to the fibers, data can be read out directly through an access panel in the skin, bypassing all NSROC hardware. Commanding is always done through the umbilical. 
%
%The science chain TM matrix is specified in the table below:\\ 
%\begin{adjustbox}{width=\textwidth,totalheight=\textheight,keepaspectratio}
%	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%		\hline
%		SF & Word 0 & Word 1 & Word 2 & Word 3 &Word 4 &Word 5 & ... & Word 120 & Word 121 & Word 122 & Word 123 & Word 124 & Word 125\\
%		\hline
%		0 & SFID & \cellcolor{yellow} sync\_a & \cellcolor{yellow} sync\_b  & \cellcolor{yellow} SFID $|$ DD & \cellcolor{yellow} MF (MSB) & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & FS1 & FS2 & FS3 & FS4\\
%		\hline
%		1 & SFID & \cellcolor{yellow} sync\_a & \cellcolor{yellow} sync\_b & \cellcolor{yellow} SFID $|$ DD & \cellcolor{yellow} MF (LSB) & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & FS1 & FS2 & FS3 & FS4\\
%		\hline
%		2 & SFID & \cellcolor{yellow} sync\_a & \cellcolor{yellow} sync\_b   & \cellcolor{yellow} SFID $|$ DD & \cellcolor{yellow} HK & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & FS1 & FS2 & FS3 & FS4\\
%		\hline 
%		3 & SFID & \cellcolor{yellow} sync\_a & \cellcolor{yellow} sync\_b   & \cellcolor{yellow} SFID $|$ DD & \cellcolor{yellow} HK & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & FS1 & FS2 & FS3 & FS4\\
%		\hline
%		4 & SFID & \cellcolor{yellow} sync\_a & \cellcolor{yellow} sync\_b   & \cellcolor{yellow} SFID $|$ DD & \cellcolor{yellow} HK & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & FS1 & FS2 & FS3 & FS4\\
%		\hline
%		... &&\cellcolor{yellow} &\cellcolor{yellow} &\cellcolor{yellow} &\cellcolor{yellow} &\cellcolor{yellow} &\cellcolor{yellow} &\cellcolor{yellow} &\cellcolor{yellow} &&&&\\
%		\hline
%		125 & SFID & \cellcolor{yellow} sync\_a & \cellcolor{yellow} sync\_b  & \cellcolor{yellow} SFID $|$ DD & \cellcolor{yellow} HK & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & FS1 & FS2 & FS3 & FS4\\
%		\hline
%		126 & SFID & \cellcolor{yellow} sync\_a & \cellcolor{yellow} sync\_b  & \cellcolor{yellow} SFID $|$ DD & \cellcolor{yellow} HK & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & FS1 & FS2 & FS3 & FS4\\
%		\hline
%		127 & SFID & \cellcolor{yellow} sync\_a & \cellcolor{yellow} sync\_b  & \cellcolor{yellow} SFID $|$ DD & \cellcolor{yellow} HK & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & \cellcolor{yellow} Pixel Data & FS1 & FS2 & FS3 & FS4\\
%		\hline
%	\end{tabular}
%\end{adjustbox}
%
%\bigskip
%
%\begin{tabular}{l|l}
%	SFID & Sub Frame ID\\
%	DD & Data Descriptor\\
%	MF & Major Frame Counter\\
%	FS & Frame Synchronization\\
%\end{tabular}
%\hspace{1 in}
%\begin{tabular}{l|l}
%	HK & Housekeeping\\
%	sync\_a  & 1$^{st}$ sync word\\
%	sync\_b  & 2$^{nd}$ sync word\\
%\end{tabular}
%\\
%
%One major frame consists of 128~minor frames, and each minor frame consists of 126 16-bit words. The science instrument will generate all words with the exception of SFID and FS (i.e., all words shaded yellow will be generated by the science instrument). The 32-bit MF counter is split across the Word 4 in SF0 (MSB) and SF1 (LSB). The MSB is Bit 0 in NSROC convention. The HK cycle is 2~major frames, while the DD cycle is 1~subframe. Data rate into the TM section is 20~Mbit/s per science chain. %Additional information on the TM format is provided in Appendix \ref{appendixB}.
%
%Each science chain has its own 28~VDC power supply in TM. In flight, the busses draw power from their associated battery (Table \ref{Batteries}). On the ground, they can also draw external power from the umbilicals. The science chains require draw a maximum current of 1.19~A. 
%
%\begin{table}[h]
%	\begin{tabular}{cccccccc}
%		\hline
%		\textbf{System} & \textbf{Voltage} & \textbf{Number} & \textbf{Cell} & \textbf{Capacity} & \textbf{Estimated} & \textbf{Load} & \textbf{Power} \\
%		& & \textbf{Of Cells} & \textbf{Type} & \textbf{Rating} & \textbf{Load} & \textbf{Duration} & \textbf{Margin} \\
%		\hline
%		Experiment X  & 28.8~V & 24 & ``F" NiCad & 7.00~Ah & 4075~mA & 1280.6~sec & 4.02\\
%		Experiment Y  & 28.8~V & 24 & ``C" NiCad & 2.3~Ah & 2550~mA & 1280.6~sec & 2.11\\
%	\end{tabular}
%	\caption{Micro-X Science Chain Power}
%	\label{Batteries}
%\end{table}
%
%	\begin{wrapfigure}{r}{0.6\textwidth}
%		\includegraphics[width=0.6\textwidth]{figs/mux.png}
%		\caption{The MUX stack} 
%		\label{MUXFigure}
%	\end{wrapfigure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{ADR Electronics}
\label{sec:ADR Electronics}

The ADR controller (ADRC) maintains a stable, cryogenic operating temperature for the detectors. The system includes the magnet power supply (to regulate power) and the ADRC stack (to run the PID loop and digitize housekeeping data). The ADR control electronics interface to the WFF93 encoder. They are based off the unit used for the XQC (\cite{mccammon2002}), with a redesigned TM interface. %There are 5 types of signals that interface to the ADR controller: \\
%
%\begin{table} [h]
	%\begin{center}
%	\begin{tabular}{llll}
%		\hline
%		\bf{Signal} & \bf{DataType } & \bf{Interface} & \bf{Details}\\
%		\hline
%		Housekeeping output & RS422 & TM & ADR HK output\\
%		Commands & 0V/5V & TM & Timer commands\\
%		LHe gauge power & 28~V & Umbilical & GSE only\\
%		LHe gauge data & 20~V & Umbilical & GSE only\\
%		Thermometry & Voltage readout & Access panel & GSE only\\
%		Filter heating & Voltage & Access panel & GSE only\\
%	\end{tabular}
	%\end{center}
%\end{table}
%\bigskip
%
%The housekeeping data is a 115.2~kbaud RS422 stream. 
The 82~kbit/s housekeeping data stream is made up of 48 serially transmitted signals to monitor the health of the system. %A buffer/driver is used in the TM section to protect the RS422 interface from accidental damage. A 120~Ohm termination resistor is required at the receiver end of the RS422 data path. 
All commands are timer-activated. %When off, the command lines are connected to the ground bus on-board. When on, they draw 5~V from a TM power bus. They may be on for several minutes. The liquid helium gauge only interfaces to the experimenter GSE through the umbilical. The thermometry and filter heating signals are connected directly to the experimenter GSE through the access panel. \\
In flight, the ADR controller sends housekeeping data to the WFF93 encoder, and the transmitted data is recorded on the ground in real time. %Timer-activated commands are sent to the controller.
%\textbf{On the rail:} The data stream that is telemetered in flight is sent through a fiber on the rail. Commands come directly through the umbilical from the experimenter GSE. External 5~V power lines are supplied on the umbilical directly from the GSE to supply power for commanding when TM is off. A duplicate set of RS422 output signals is provided for night operations. For night operations with 36.245, the TM1 power bus had to stay on to use these lines to keep the buffer in TM powered on. 

The ADR requires 28~VDC power. ADR power is supplied from both power busses with a diode-or circuit to supply power even if one of the power busses fails. The magnet power supply can drive the superconducting magnet with up to 9.4~A of current. %Once the magnet is energized, the power supply to the ADR must not be interrupted at all (this includes operations like switching from external to internal power). \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Laser Position Monitor Interface: P983}
%
%The laser positioning system monitors the position of the cryostat with respect to the rocket skin by reading out the position of two laser beams on two photosensors. The laser electronics interface to the TM1 link. This system has two types of signals: \\
%
%\begin{table} [h]
	%\begin{center}
%	\begin{tabular}{llll}
%		\hline
%		\bf{Signal} & \bf{DataType } & \bf{Interface} & \bf{Details}\\
%		\hline
%		Power/grounds & 28~V & TM & Sourced from PBX\\
%		Output & RS422 & TM & Position data\\
%	\end{tabular}
	%\end{center}
%\end{table}
%\bigskip
%
%The RS422 output is 115.2~kbaud with no flow control, 8~bit data words, 1 start bit, 1 stop bit, and no parity. A 120~Ohm termination resistor is required at the receiver end of the RS422 data path. A buffer/driver is used to protect the RS422 interface. \\
%\textbf{In flight:} The Position Monitor output is sent to the TM1 encoder. \\
%\textbf{On the rail:} The data stream that is telemetered in flight is sent through a fiber on the rail. There are no umbilical connections and no uplink. \\
%\begin{wrapfigure}{r}{0.7\textwidth}
%	\includegraphics[width=0.7\textwidth]{figs/adrc.png}
%	\caption{The ADR Control Electronics} 
%	\label{MUX}
%\end{wrapfigure}
The ADRC holds the Housekeeping A/D and TM Interface board (TMI), the Miscellaneous Housekeeping board (MHK), the GRT Readout board (GRT), the Digital Sine and PID Controller board (PID), the Magnet Drive and LHe gauge board (Mag Drive), and the Command Buffers board (CMD). The magnet and LHe gauge are controlled by the Mag Drive board. The control loop for the ADR temperature is driven by the GRT and PID boards: the GRT board reads out the two GRTs on the FEA, while the PID board controls the PID loop. The MHK board monitors temperatures and voltages from the other boards. The TMI board reads analog voltages from the other cards, digitizes them and multiplexes them into the serial asynchronous RS422 stream. The CMD board buffers the RS422 stream from the TMI board and sends it directly to TM. It also receives commands from TM flight timers to ramp up the magnet, ramp down the magnet, set the GRT mode (high or low mode via the stimulus current on the thermometers), and set the magnet ramp speed. 
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Valve Controllers}
\label{sec:Valve Electronics}
%
%The gate and pumping valves use identical control boxes, specifically designed for Micro-X, that are mounted inside the payload. Different firmware is programmed for the gate valve and pumping valve microcontrollers to satisfy the specific needs of that valve. 
%
%The heat switch motor control box is a commercial controller from Hayden-Kerk (model DCS 4020) that does not fly. The heat switch is only actuated on the ground.

Two valves are used for flight operations: the OTD valve to expose the detectors to X-rays, and the BTS valve to open the He bath to space for pumping. Each valve is driven by its own on-board microcontroller receive timer commands from TM, issue commands to the motor, read out limit switches, and measure both current draw and local pressure. The OTD measures the pressure in the optics section, and the BTS measures the pressure in the He bath. The microcontrollers are the same board, but with different firmwares. %The output from these systems can be read at the minimum sampling rate. All digital inputs on the controllers have a 100~kOhm pull-down resistor.
%The gate valve controller runs the gate valve on the aft end of the hermetic bulkhead. 
%It has four types of signals: \\
%
%\begin{table} [h]
	%\begin{center}
%	\begin{tabular}{llll}
%		\hline
%		\bf{Signal} & \bf{Data Type } & \bf{Interface} & \bf{Details}\\
%		\hline
%		Power/grounds & 28~V & TM & Soured from PBX\\
%		Commands & 5V & TM & Timer commands\\
%		Analog output & 0-5~V & TM & Current monitor\\
%		Analog output & 0-10~V & TM & Vacuum gauge output\\		Digital output & 5~V & TM & Limit switches\\
%		Digital output & RS422 & Umbilical & GSE only
%	\end{tabular}
	%\end{center}
%\end{table}
%
%\bigskip
%The gate valve system has a controller, a motor and a vacuum gauge. %%%%%%%%The gauge requires 28~VDC power and outputs an analog voltage (0-10~V). Its output is fed through a voltage divider (10k series, 6.81k shunt, Vout = 0.405~Vin) in TM to scale it down to the 0-5~V range accepted by the PCM encoder analog input. %This allows a maximum vacuum gauge output of 12.3~volts. 
Both the OTD and BTS controllers require 28~VDC power, accept 5~V digital commands as inputs, and output HK data. %The optics gate valve controller requires 28~VDC, accepts four 5~V digital commands, and outputs HK data. %both analog (current monitor) and digital (limit switches) data. The vacuum gauge requires 28~VDC and outputs analog data. %Its output is both digital (limit switches) and analog (current monitor). 
In flight, they is commanded by timers and output data to TM1.  
%\textbf{On the rail:} The data that is telemetered in flight is sent through a fiber on the rail. An RS422 stream is sent down the umbilical to the experimenter GSE. Commands are sent through the umbilical.\\
%\bigskip

\com{I took out heat switch since it isn't a valve. Do we need/want to say anything more about our heat switch?} 
%The output from these systems can be read at the minimum sampling rate. All digital inputs on the controllers have a 100~kOhm pull-down resistor.
%The gate valve controller runs the gate valve on the aft end of the hermetic bulkhead. 
%It has four types of signals: \\
%
%\begin{table} [h]
	%\begin{center}
%	\begin{tabular}{llll}
%		\hline
%		\bf{Signal} & \bf{Data Type } & \bf{Interface} & \bf{Details}\\
%		\hline
%		Power/grounds & 28~V & TM & Soured from PBX\\
%		Commands & 5V & TM & Timer commands\\
%		Analog output & 0-5~V & TM & Current monitor\\
%		Analog output & 0-10~V & TM & Vacuum gauge output\\		Digital output & 5~V & TM & Limit switches\\
%		Digital output & RS422 & Umbilical & GSE only
%	\end{tabular}
	%\end{center}
%\end{table}
%
%\bigskip
%The gate valve system has a controller, a motor and a vacuum gauge. %%%%%%%%The gauge requires 28~VDC power and outputs an analog voltage (0-10~V). Its output is fed through a voltage divider (10k series, 6.81k shunt, Vout = 0.405~Vin) in TM to scale it down to the 0-5~V range accepted by the PCM encoder analog input. %This allows a maximum vacuum gauge output of 12.3~volts. 
%\textbf{On the rail:} The data that is telemetered in flight is sent through a fiber on the rail. An RS422 stream is sent down the umbilical to the experimenter GSE. Commands are sent through the umbilical.\\
%\bigskip

%The pumping valve controller runs the valve on the avionics skin. 
%It has four types of signals: \\
%
%\begin{table} [h]
%	%\begin{center}
%	\begin{tabular}{llll}
%		\hline
%		\bf{Signal} & \bf{Data Type } & \bf{Interface} & \bf{Details}\\
%		\hline
%		Power/grounds & 28~V & TM & Sourced from PBX\\
%		Commands & 5~V & TM & Timer commands\\
%		Analog output & 5~V & TM & Current monitor\\
%		Analog output & 0-5~V & TM & Pressure gauge\\
%		Digital Output & 0~V/5~V & TM & Limit switches\\
%		Digital output & RS422 & Umbilical & GSE only
%	\end{tabular}
	%\end{center}
%\end{table}
%
%\bigskip
%The pumping valve system has a controller, a motor and a pressure gauge. 
%The LHe tank gate valve controller requires 28~VDC, accepts 3 commands, and outputs HK data. %both analog (current monitor) and digital (limit switches) data. The pressure gauge requires 28~VDC power and outputs analog data. 
%both digital (limit switches) and analog (current monitor). 
%In flight, the pumping valve system is commanded by timers and outputs HK data to TM1. 
%\textbf{On the rail:} The data that is telemetered in flight is sent through a fiber on the rail. An RS422 stream is sent down the umbilical to the experimenter GSE. Commands are sent through the umbilical. %Wirelists are provided in \S \ref{Wirelists}. \\

%\subsubsection{NSROC Systems Interfaces}
%\label{sec:NSROC Electricals}
%A NSROC-supplied shutter door, CDI, vibrometers and star tracker are located in the science instrument. Harnessing runs from these components, past the science instrument, and out to TM. Six vibrometers are mounted in the science instrument:  Skin Thrust Axis, Skin Lateral, ADR Thrust Axis, ADR Lateral, Mirror Thrust Axis and Mirror Lateral. Each vibrometer has a charge amplifier and passes through an anti-alias filter. %A minimum Nyquist frequency of 3~kHz is required. Each vibrometer has a charge amp, and the amplified signals are fed into the anti-alias filters on the interface plate between the science instrument and TM. The anti-alias filters read out directly to TM. %Four vibrometers are in the vented section, and their harnessing runs directly to TM. The harnessing for the two vibrometers in the optics section pass through the hermetic bulkhead, on the same connector as the star tracker. 
%\end{itemize}
%\begin{figure} [htp]
%\begin{center}
%\vcenteredhbox{\includegraphics[width=0.75\textwidth]{figs/bulkhead.png}}
%\end{center}
%\caption{Star Tracker bulkhead connection} 
%\label{WireMap}
%\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Experiment Umbilical}
%\label{Umbis}
%The power, commanding and readout of the science instrument must be accessible when all payload sections are mated to each other, including on the rail. Umbilical signals can be used to run detectors overnight. %Any signals required when TM is off are connected to either the railside rack or the umbilicals. 
%ADR magnet power can be supplied through the umbilical to maintain continuous power when the magnet is on during the launch countdown. 
%
%The experimenter GSE connections to the umbilical are listed provided in \S \ref{Wirelists}. % and Figure~\ref{UmbiSchematic}. \\
%\begin{figure} [htp]
%	\begin{center}
%		\vcenteredhbox{\includegraphics[width=\textwidth]{figs/gse_umbi.pdf}}
%	\end{center}
%	\caption{Umbilical connections}
%	\label{UmbiSchematic}
%\end{figure}
%
%\subsection{Access Panel}
%\label{APSection}
%Four connectors from the science instrument interface to an access panel on the rocket skin: \\
%
%\begin{table} [h]
%\begin{center}
%	\begin{tabular}{llll}
%		\bf{Connector} & \bf{Connector} & \bf{Signals} & \bf{Data Type}\\
%		\bf{Name} & \bf{Type} & & \\
%		\hline
%		APX-MCB-J3 & HD44 & Science Chain X & LVDS downlink; RS422 and 5~V uplink; clocks \\
%		APY-MCB-J3 & HD44 & Science Chain Y & LVDS downlink; RS422 and 5~V uplink; clocks\\
%		AP-CRY-J1 & SD37 & M79 Thermometry & VDC input and output\\
%		AP-BTS-J1 & SD9 & Pumping valve heaters & VDC input\\
%	\end{tabular}
%	%\end{center}
%\end{table}
%These connectors interface to a railside rack, and they interface to NSROC to supply power to the railside rack. The rack will contain one computer, two power supplies, three readout boxes, and one bridge. It will sometimes hold the two science chain GSE (telemsim) boxes. The rack will be removed directly before final arming. 
%
%Each of the science chain connectors will interface to its own telemsim box. These boxes receive the full speed LVDS downlink ($\sim$66~Mbit/s) and convert the data to USB, which runs via fiber to a fiber converter in the mini blockhouse, then run through the trench to the blockhouse. The telemsim and USB converter boxes both require wall power. In addition to the downlink, the telemsim boxes supply the required clocks to the MUX stacks when the encoders are not connected. 
%
%The third access panel connector receives and reads out thermometry signals from the cryostat onto the computer on the rack. 
%
%The fourth connector supplies power to heating resistors on the pumping valve. 

==> sections/flight-livetime.tex <==
DEPRECATED!!!!!!

\subsection{Livetime}
\label{sec:Livetime}

As mentioned in \S \ref{sec:flight-overview}, in addition to the loss of target from the ACS failure, we observed periods of time during the science observation where no TES pulses were recorded. During these periods, the SQUID readout had ``lost lock" in those channels and no signals from the TES were recorded. The SQUIDs are read out via a feedback loop which is ``locked" to a particular set point. Some of SQUID readouts drifted beyond their stable set points and ``lost lock" for portions of the flight due primarily to interactions between the SQUIDS and Earth's changing magnetic field direction as the payload spun. Figure~\ref{fig:Pulse_times} shows each pixel of the Micro-X TES array as a row along the y-axis, with triggered events shown as dots vs time on the x-axis. The pixels are arranged in groups of 16 corresponding to each SQUID MUX column in the 8x16 MUX system.  The times where no triggering was seen are evident in this figure, and some correlation between rows is also evident. 

\begin{figure}
	\begin{center}
		\includegraphics[width=.7\textwidth]{figs/Pulse_times_combined.png}
	\end{center}
	\caption{Timestamps of X-ray triggers vs.~time during flight. The array is separated into SQUID readout columns labeled XA--XD and YA--YD. The number in the y-axis corresponds to the SQUID channel (0--15) in each column (\S~\ref{sec:FEA}). Most of the triggers are from the on-board calibration source. This plot indicates times during the flight that the detector readout system was considered live for each pixel.\hl{to be remade to match formatting of figure 27.} \acom{Update with energy cut to easily explain what the data is}}
	\label{fig:Pulse_times}
\end{figure}

Table~\ref{tab:livetime} shows the fractional livetime averaged per column and the exposure per column during the science observation window. This is only considering the science observation window (between 150 and 430 secs in flight), with known dead pixels included in the calculation. If all 128 pixels were live for the full 280~s observation the total exposure would be 35840~pixel$\cdot$sec. Due to the loss of lock of the SQUIDs, a total exposure of 13644.33~pixel$\cdot$sec was obtained, which is 38.07\% of the science goal. 

\begin{table}
\begin{center}
\begin{tabular}{ |c|c|c| } 
 \hline
 Column & Avg LT [\%] & Exposure [pixel$\cdot$sec]\\ 
  \hline
 XA & 1.17 & 52.66 \\  
 XB & 26.65 & 1198.33 \\ 
 XC & 18.19 & 817.97 \\ 
 XD & 29.57 & 1329.37 \\
 YA & 23.04 & 1035.97 \\  
 YB & 62.08 & 2791.14 \\ 
 YC & 55.42 & 2491.42 \\  
 YD & 87.36 & 3927.47 \\ 
   \hline
 Total & 37.94 & 13644.33 \\ 
 \hline
\end{tabular}
 \caption{Fractional livetime averaged per column and the exposure per column during the science observation window.}
 \label{tab:livetime}
\end{center}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PIXEL Livetime
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Figure~\ref{fig:sideXlivetime} shows fractional livetime of side X during observation.
% Figure~\ref{fig:sideYlivetime} shows fractional livetime of side Y during observation.

% \begin{figure}
% 	\begin{center}
% 		\includegraphics[width=0.7\textwidth]{figs/Livetime_SideX_observation.png}
% 	\end{center}
% 	\caption{Fractional livetime of each pixel on side X during the science observation window.}
% 	\label{fig:sideXlivetime}
% \end{figure}

% \begin{figure}
% 	\begin{center}
% 		\includegraphics[width=0.7\textwidth]{figs/Livetime_SideY_observation.png}
% 	\end{center}
% 	\caption{Fractional livetime of each pixel on side Y during the science observation window.}
% 	\label{fig:sideYlivetime}
% \end{figure}

\subsubsection{Magnetic Fields During Flight}

\begin{figure}
	\begin{center}
		%\includegraphics[width=0.7\textwidth]{figs/mag_temp.png}
		\includegraphics[width=\textwidth]{figs/flight_mag.png}
	\end{center}
	\caption{A three-axis magnetometer showed the rocket spinning in the Earth's field during powered flight (region 1). The payload slowly tumbled for the duration of the science observation (region 4) due to the ACS failure. The large changes in magnetic field during the rocket descent are characteristic of sounding rocket descents; their source has not been confirmed, but it is not dominated by the Earth' field.}
	\label{fig:Magnetometers}
\end{figure}


The loss of SQUID lock during flight in some channels is attributed to the interaction between the magnetic field environment and the SQUIDs.
Under a nominal flight, the magnetic field around the payload is relatively constant during the science observation while the payload is pointing at its science target. For the Micro-X flight, however, the slowly rotating payload meant that the direction of the magnetic field as seen from the rocket was continually changing during science observation, as shown in the region marked ``4" in Figure~\ref{fig:Magnetometers}. The magnetic field encountered in flight was measured by the three-axis magnetometer in the telemetry section. The response of the magnetometers is in good agreement with projection of the Earth's field from the rocket trajectory, as derived from the International Geomagnetic Reference Field (IGRF) model~\cite{IGRF}. %As discussed in \S\ref{sec:Shielding}, the response of both SQUIDs and TESs are affected by magnetic flux. The impact of the magnetic field on the SQUIDs and TESs is described in \S\ref{sec:SQUID_magnetic_susceptibility} and \S\ref{sec:TES_magnetic_susceptibility}, respectively. 
Figure~\ref{fig:Magnetometers} also shows the effect of the rotation during ascent on the measured magnetic field (region 1), and the unstable readings during re-entry and parachute descent (regions 6 and 7) which is nominal for magnetometers during these phases of flight.
 %The parachute descent does not offer additional information on the SQUID response because the magnetic field in this period is unstable and unpredictable. In this portion of the flight, the projected magnetic field from the Earth's field deviates from the observed field in the magnetometer, and the SQUID response no longer tracks the Earth's field in the direction of the Nb can holes. This unstable magnetic field is a known phenomenon in sounding rocket flights. \acom{Can we get a real citation for this?} Its exact origin is unknown, but it is hypothesized that the hot rocket skin breeds a plasma around the rocket as it descends, creating an unpredictable and unmodeled magnetic field environment. This unpredictable environment is empirically confirmed by both the magnetometer and SQUID responses. \rcom{putting the direct quote from Adam Blake's engineer "There is a tremendous amount of heat generated during re-entry that may have caused some plasma generation and generated a corresponding magnetic moment which may have affected the sensed field. There are typically ferrous metals in the payload and these may lense the sensed magnetic field depending upon the payloads attitude."}

\subsubsection{SQUID Response}

%The primary cause of the lost live-time during flight is believed to be due to \tcom{the drifting baseline of the SQUID response due to the interaction of changing magnetic field around the superconducting shield from the unintended tumbling of the payload during flight (Sec.~\ref{}\tcom{add ref})} the coupling between Earth’s magnetic field and the SQUIDs. 
Both the SQUIDs and TES are shielded from magnetic fields by a superconducting Nb can surrounding the detector housing (\S \ref{sec:FEA} and \ref{sec:Shielding}). The flown NIST MUX06a multiplexing readout system (\S \ref{sec:FEA}) is known to be particularly susceptible to magnetic fields due to the high effective area of the SQ2 summing coil~\cite{Stiehl:2011}, which is more than two orders of magnitude larger than the SQ1 effective area. A relatively small change in the field at the SQ2 summing coil can dramatically change the relationship between the three SQUID stages. This manifests as a change in the locked feedback baseline, and if the drift is significant enough it may become impossible to null out the SQ1 flux input as described in \S \ref{sec:FEA}. When this happens, the SQUIDs would be “unlocked” and unable to read out the detectors. This effect can be tracked by looking at the locked feedback baseline of the TESs during observation and powered flight.

\begin{figure}
	\begin{center}
		\includegraphics[width=0.7\textwidth]{figs/temp-poweredflight-baseline.png}
	\end{center}
	\caption{Magnetic field in the X-direction during \hl{powered flight} (top), as measured by the on-board magnetometer. Any impact from magnetic fields is due to the SQUID susceptibility because the TESs are normal in this period. The baseline of the locked SQUID feedback signal (bottom) was strongly negatively correlated with the Earth's magnetic field in the X-direction. \hl{The correlation between the SQUID response and external field continues after the rocket goes through its de-spin mechanism at roughly T+63~s. } \hl{Remake, add more pixels, and x-axis time.} \acom{Show de-spin}}

	\label{fig:powered_flight}
\end{figure}

The ADR refrigerator is launched at a temperature of 300~mK to increase its heat capacity during powered flight (\S \ref{sec:Operations}). At this temperature the TESs are in their normal state, thus during powered flight the TES detectors behave like resistors in the SQUID readout circuit and have no sensitivity to changing magnetic fields. During powered flight the rockets spins at up to 4.5 Hz for stability, causing a rotation of Earth’s magnetic field relative to the payload. Figure~\ref{fig:powered_flight} shows the locked feedback baseline during powered flight for example pixels. The SQUID feedback signal shows strong anti-correlation with the magnetic field in the x-axis. \acom{Need statement or resolution of timing offset between sides.} The rocket x-axis is close to the orientation of the readout wiring holes in the Nb magnetic shield (Figure~\ref{Nb-Shield-with-Magnet}). This suggests that the rotating external magnetic field couples most strongly to the SQUIDs inside the Nb shield through these holes.

%Similar effects are \tcom{tense: present or past?} observed during powered flight when the TESs are normal. During powered flight the rockets spins at up to 4.5 Hz for stability, causing a rotation of Earth’s magnetic field relative to the SQUIDs. The locked feedback baseline again tracks Earth’s magnetic field in the rocket-x-direction confirming that this is a SQUID effect and not a TES effect.  However, during powered flight there some complications due to the system having been tuned at 75mK but launched at 300mK. These complications are discussed in more depth in \hl{[cite LTD19 proceedings]} \tcom{These complications... is very vague. What exactly do you mean, can we say something more concrete?}.\jcom{The previous two sentences are to point the reader towards the LTD conference proceedings for a more in-depth look at the effects of magnetic field on the squids. Stuff like some columns being 180 degrees out of phase during powered flight because they locked on the slow side.} 

During the science observation, the payload tumbled with an average rate of 1.6 degrees/s, and a maximum rate of 4.7 degrees/s due to the ACS pointing failure. Figure~\ref{fig:squids_science_obervation} shows the baseline of several pixels vs. time, along with the magnetometer reading along the rocket-x axis. As during powered flight, a strong correlation is seen between the two signals. For some pixels, the SQUIDs unlock when the magnetic field in the rocket-x direction is near its maximum value.  The SQUIDs did not all unlock simultaneously, likely due to small variances in the SQUID properties and tune and the complex magnetic field distribution inside the superconducting shield. However, most pixels within a single TDM column behaved similarly, consistent with the SQ2 coupling hypothesis. This behavior appeared for the first time in flight; it was not observed in laboratory operations or in ground operations in the days before launch. %As a result of this unlocking, the science observation had an exposure equivalent to 118 seconds of the full array.
Modeling of the SQUID lock loop response to baseline changes has been able to reproduce the major features of this data and can reproduce the unlocking behavior seen during flight~\cite{Fuhrman:2021}. 


\begin{figure}
	\begin{center}
		\includegraphics[width=0.7\textwidth]{figs/temp-observation-baseline.png}
	\end{center}
	\caption{The baseline of the SQUID feedback signals tracked the external magnetic field in the X-direction during the science observation, consistent with the powered flight response. Those portions where the baseline signal disappears are due to the pixel becoming unlocked, as described in the text. \acom{Convert into a scatter plot; rename "SQ1 lcoked feedback" to what's used in the paper - maybe "Locked Baseline [uA]"?}}
	\label{fig:squids_science_obervation}
\end{figure}

\subsubsection{Post-flight Tests}

The magnetic susceptibility of the SQUIDs was measured with post-flight Helmholtz coil testing. Two coils in a Helmhlotz configuration were placed along three orthogonal axes (one axis measured at a time) around the exterior of the rocket skin. An external DC magnetic field was incrementally applied with the instrument in different configurations. By performing these tests with only the SA biased, the test confirmed that SAs were not discernibly susceptible to picking up external field. Next, the SQ1s and SQ2s were biased. The baseline of the signal was seen to change in correlation with the applied external field. Incremental changes in the signal baseline due to the applied external field could be offset by incremental changes to the SQ2 flux bias, effectively canceling the effects of the external field and supporting the idea that the SQ2 summing coil is the primary coupling point. By contrast with the SA tests, when biasing the entire 3-stage SQUID readout, a significant fraction of the SQUIDS reliably unlocked at high fields. The composite SQUID response also showed a significant dependence on the speed of the magnetic field change (dB/dt). When the applied field was rapidly increased, then decreased slowly, the SQUID response did not return to its original position but showed a significantly hysteretic response. However, the field rate of change needed to cause this hysteretic effect is much higher than what we observed in flight. These measurements indicate that 0.3\% to 1\% of external fields applied across the SQUID plane couple to the SQ2, while only 0.1\% of external fields applied perpendicular to the SQUID plane do. The magnitude of the response shows correlation to SQUID columns, with the response of SQUID column A$>$B$>$C$>$D, explaining why YD spent the most time locked. It takes less than 1/4 of a SQ2 $\Phi_0$ to unlock the SQUIDs in most situations, corresponding to only 11~mG at the SQ2 summing coil. Tumbling through Earth’s magnetic field could therefore be sufficient to unlock the SQUIDs. 

\hl{After it was determined that the SQUIDs operated during the first flight were indeed susceptible to an external magnetic field, they were swapped to a less susceptible model (\S\ref{sec:Reflight}). Helmholtz coils were again used to sweep the external electric field from approximately -600~mG to 1200~mG (ambient field in the laboratory was $\sim$300~mG). The SQUIDs remained locked, indicating that the magnitude of the Earth's magnetic field is no longer enough to cause the readout to lose lock. A separate test proved that the rate of the changing magnetic field also does not cause unlocking, as the magnetic field was rapidly oscillated at $\sim$4~Hz. Finally, the external magnetic field sweep was repeated with the TESs in both normal and superconducting states; this also did not result in any unlocking. This series of tests validates the theory that the TESs were not responsible for the unlocking issues experienced during the first flight and the magnetic field was indeed coupling to the SQUIDs.}

%The magnetic susceptibility of the SQUIDs to the Earth's field in flight was measured by tracking the evolution of the \hl{baseline and the untriggered feedback signal} in the detector response. As described in \S\ref{sec:Operations}, the SQUIDs were biased before flight. The SQUIDs and TESs launched at 300~mK, and the TES were therefore normal. The ADR began regulating the system to 75~mK after powered flight. A combination of data from powered flight -- which isolates the SQUID response to external fields -- and the science observation provide a consistent evaluation of the flight susceptibility. 

%During powered flight, the rocket was spinning in the Earth's magnetic field at up to 4.5~rotations/s, as measured by the on-board magnetometer (\S\ref{sec:flight_magnetic_field}). The SQUID response during powered flight tracked the magnetic field response, indicating a susceptibilty in the SQUIDs as the TESs were normal. The external field is believed to couple the strongest to the SQ2 stage, which has an effective area that is nearly two orders of magnitude larger than the SQ1 stage (\S\ref{sec:FEA}). The MUX06a SQ2s used in the first flight are known to be particularly susceptible to external magnetic fields~\cite{Stiehl:2011}. The correlation was strongest in the direction of the holes in the superconducting Nb shield, which are required to pass through the harnessing to the FEA, as shown in Figure~\ref{fig:fea}. Figure~\ref{fig:powered_flight} shows the magnetic field in this direction along with the instrument response (\hl{untriggered feedback signal}) during powered flight. 

%After powered flight, the rocket de-spinning mechanism slowed the spinning of the payload. The ADR began to regulate temperature, and the TES were moved into their superconducting transition for the science observation. During the science observation, the payload spun with an average roll rate of 1.6$^\circ$/s, and a maximum rate of 4.7$^\circ$/s. While the detectors began to see X-rays from the on-board calibration source, the baseline of the SQUID response continued to track the Earth's field in the direction of the holes in the Nb can, as shown in Figure~\ref{fig:squids_science_obervation}. This behavior is qualitatively consistent with models simulating the response of the 3-stage SQUID readout to external magnetic fields. \acom{Add full science observation analysis here}

%The external magnetic field moved some SQUIDs far enough from their operating points that they ``unlocked." This means that they deviated enough from their operational settings that their feedback loops were unstable and they effectively stopped reading out. This unlocking is a result of the Earth's field coupling into the SQUIDs while the payload spun. Under a normal flight trajectory, the payload would have been effectively stationary during the science observation. Due to the ACS failure, the payload continued to tumble throughout the science observation, so the SQUIDs continued to experience a changing field. The unlocking was not instantaneous across the entire array, as shown in Figure~\ref{fig:unlocking}. It did broadly track by TDM column, consistent with the SQ2 driving the effect. This behavior appeared for the first time in flight; it was not observed in laboratory operations or in ground operations in the days before launch. As a result of this unlocking, the science observation had an exposure equivalent to 118 seconds of the full array. 

% \begin{figure}
% 	\begin{center}
% 		\includegraphics[width=0.5\textwidth]{figs/temp_unlocking.png}
% 	\end{center}
% 	\caption{The changing external magnetic field led to a number of SQUIDs unlocking in flight. Each dot here is a triggered X-ray of at least \hl{1~keV}. \hl{Will be updated: black points, single plot, energy cut implemented}}
% 	\label{fig:unlocking}
% \end{figure}

%The SQUIDs' magnetic susceptibility was measured with post-flight Helmholtz coil testing. Two coils in a Helmhlotz configuration were placed along three orthogonal axes (one axis measured at a time) around the exterior of the rocket skin. The spinning of the Earth's field around the rocket's reference frame during powered ascent was approximated by applying a sinusoidal magnetic field profile using the Helmholtz coil in the x and y rocket coordinate directions one axis at a time. By performing this test with only the SA biased, the test confirmed that SAs were not discernibly susceptible to picking up external field, indicating successful magnetic shielding at the SAs. By contrast, when biasing the entire 3-stage SQUID readout \tcom{can we say we biased just the SQ2 and SA? Did we do that, with the SQ1 off?}, a significant fraction of the SQUIDS reliably unlocked. The composite SQUID response showed a significant dependence on both field strength and the speed of the magnetic field change (dB/dt). A gradual progression up to one Earth field moved the average composite SQUID response by \hl{0.1$\Phi_0$}, where $\Phi_0$ represents one period in the oscillatory SQUID response. By contrast, a discrete jump from no field to three Earth's fields shifted the average composite SQUID response by \hl{0.7$\Phi_0$}. When the Helmholtz coils returned to zero field, the SQUID response did not return to its original position, but showed a significantly hysteretic response. This hysteresis complicates comparisons to flight data. The susceptibility in the direction of the holes in the Nb shield was not probed directly; the closest measurement was clocked 22.5$^\circ$ from that direction \rcom{can we get a final answer if this was CW or CCW- so that we know if this is towards or away from the x-axis}. This was the most susceptible of the measured directions, consistent with the flight observation that the most susceptible direction was that of the Nb shield holes \tcom{you mean the rectangular readout cable holes? Let's be specific. We should have that pointed out in the magnetic shield section and add it here}. These measurements indicate that the magnetic shielding protected the SQUIDs from 99.0--99.9\% of incident external field, with 99.0--99.3\% effective shielding in the direction of the Nb shield holes. \hl{This corresponds to an incident field at the SQUIDs of 44~mG in flight.}


%COMSOL 

\begin{figure}
	\begin{center}
		\includegraphics[width=0.9\textwidth]{figs/ComsolModel4Panes.png}
	\end{center}
	\caption{COMSOL models the remnant field inside the Nb shield for an external magnetic field of 0.5~Gauss was applied in the snout axis (top), perpendicular to the snout axis (center), and the thrust axis (bottom). These axes are rotated from the magnetometer and Helmholtz axes, shown in the top left figure, by 22.5$^\circ$. The octogonal outline of the FEA is shown in the center of the Nb shield. As SQUID coupling is the strongest in the thrust axis, results are shown at the X-Y plane of the SQUID and TES chips for the total magnetic field (left) and the thrust axis (right).  \acom{Font/size should match other figures; how does this look in black/white - look into the monosomething color schemes; add Z axis}
	}
	\label{fig:COMSOLmodel}
\end{figure}

\begin{table}
\begin{center}
\begin{tabular}{ |c|c|c|c|c| } 
    \hline
    Column & Total Residual Field [Gauss] & Residual Field in Z-direction [Gauss] & Total Shielding Factor & Z-Direction Shielding Factor\\
    \hline
    XA & 8.4E-04 & 1.3E-04 & 590 & 3,900\\  
    XB & 7.4E-04 & 8.3E-05 & 680 & 6,000\\ 
    XC & 6.8E-04 & 3.0E-05 & 730 & 17,000\\ 
    XD & 6.9E-04 & -4.6E-05& 720 & 11,000\\
    YA & 8.8E-04 & -1.3E-04& 570 & 3,700\\  
    YB & 7.5E-04 & -9.7E-05& 670 & 5,100\\ 
    YC & 7.1E-04 & -3.2E-05& 710 & 16,000\\  
    YD & 7.0E-04 & 3.7E-05 & 710 & 14,000\\ 
    \hline
\end{tabular}
\caption{The residual field and shielding factor for both the total field and the field in the rocket-z direction was evaluated at each detector column for 0.5 Gauss applied in Snout direction in COMSOL. \acom{As shown, these come across as trusted numbers rather than general trends. Don't think we can trust them as well as it seems- can we add error bars or make it clear these aren't precise values?}}
\label{tab:comsol}
\end{center}
\end{table}

In addition, a model of the Nb magnetic shield was made using COMSOL Multiphysics software, where the applied magnetic field could be entered in Cartesian coordinates that matched the magnetometer data coordinates. The Nb can was simulated as two separate pieces (the lid and the cone) with thin, solid connections to replicate the lead zipper tabs. The shielding factor as well as the most susceptible direction was investigated. The Nb can was set as a ``magnetic insulation boundary" in COMSOL~\cite{Bergen2016}. A rendering in COMSOL of the Nb shield is shown in Figure~\ref{fig:COMSOLmodel}. Modeling the actual internal field configuration during flight is non-trivial due to the complex geometry of the Nb can, the changing direction of the external field, the off-axis location of the SQUIDs in the FEA, the possibility of trapped flux in the Nb, and the possibility that some of the lead zipper tabs were not fully superconducting.

The SQUID MUX chips are mounted in the rocket x-y plane inside the FEA. Thus it is expected that the z-component of fields in the z-axis at the SQUIDs will have the highest coupling to the SQUID loop area. The Nb Shield was designed such that an applied Earth's magnetic field in the z-direction results in the highest shielding factor and lowest residual field at the detectors for both total magnetic field and the magnetic field in the z-direction. Assuming the lead tabs are all connected, the worst shielding factor for total magnetic field at the SQUIDs is for external fields perpendicular to the ``snouts" of the Nb can. The snout direction is 22.5 degrees from the rocket-x axis; perpendicular to the snout is 112.5 degrees from rocket-x direction. The worst shielding factor for the z-component of the magnetic field at the center of the SQUIDs is for external fields in the x-y plane oriented at 52.5 clockwise from rocket-y direction. Figure~\ref{fig:COMSOLmodel} shows the COMSOL simulation for the total magnetic field and z-component of the magnetic field when the applied field is in the direction of the snouts and perpendicular to the snouts. 

When the Earth's field is applied perpendicular to ``snouts" of the Nb can, detector side X sees a different polarity in the magnetic field in the z-direction than detector side Y. This could explain why the baselines, and therefore the SQUIDs being locked, are not always the same between the two detector sides. 



==> sections/flight-optics.tex <==
% !TEX root = ../instrument_paper_revB.tex

\subsubsection{Pre- and Post-Flight Optics Performance}
\label{flight-optics}

Although it was not possible to evaluate the optics performance in flight without time on target, pre- and post-flight measurements were performed. The angular resolution of the X-ray mirror was measured before flight, using a 1.5~keV X-ray beam. It is expressed as the Half-Power Diameter (HPD), which encloses 50\% of all focused X-rays. After correcting for beam divergence, the angular resolution of the X-ray mirror was measured at the 2.144~m focus of the mirror to be 140~arcseconds HPD, as shown in Figure~\ref{fig:optics_alignment} (left). The alignment error budget was 2.5~arcminutes in flight. Pre-flight vibration testing was used to verify the alignment stability of the X-ray mirror to the center of the aperture valve under flight vibration conditions. The alignment of the mirror to the aperture valve shifted by 1~arcminute, and the alignment of the star tracker to the flat reference mirror shifted by 0.5~arcminutes under a launch vibration load, meeting the alignment stability requirement. Post-flight analysis of the X-ray mirror, shown in Figure~\ref{fig:optics_alignment} (right), indicated a 30~arcsecond degradation in the angular resolution, likely due to the force of impact. This degradation is consistent with expectation and is small enough that the mirror can be used for subsequent flights. 

\begin{figure}
		\begin{center}
		\includegraphics[width=0.9\textwidth]{figs/postflight_optics.png}

		\caption{X-ray mirror angular resolution before (left) and after (center) flight. The heat map images show the photon distribution at the focus of the mirror during beam tests. The right image converts these distributions to an Encircled Energy Fraction (EEF), which is the fraction of photons that fall within a circle of a given radius. The EEF shows that the Half Power Diameter of the optics was not significantly affected by the flight. }
		\label{fig:optics_alignment}
		\end{center}
	\end{figure}

==> sections/flight-preflight.tex <==
% !TEX root = ../instrument_paper_revB.tex
\subsection{Pre-flight Countdown Performance}
\label{Preflight}

All operations and instrument performance were nominal during the pre-flight countdown. %As described in \S \ref{sec:Operations}, the majority of pre-flight operations are used to prepare the ADR for flight, and both cryostat and ADR performance during the countdown were nominal. 
Table \ref{table:countdown} describes the planned operations, while Table \ref{Countdown} reports operations as they happened and includes the thermal performance of the instrument. Thermal performance is measured by the temperature of the LHe bath, the temperature of the FEA on the detector array, and the ADR magnet current (Figure~\ref{countdown-thermals}). The countdown began by filling the LHe tank, and the bath was then pumped on continuously until the LHe pumping valve was close for launch at T-6~min. The entire payload (with the exception of the external LHe bath pump) was powered off for rocket arming, and during this time, the launcher rose from 7$^\circ$ from the ground to its launch angle of 85$^\circ$. The ADR magnet cycle then began and cooled the cold stage to 75~mK for detector tuning. Detector tuning included three ``de-Gaussing cycles," in which the ADR is ramped up to 300~mK and back down to 75~mK, to minimize any hysteresis in the SQUIDs due to changing magnetic fields. It was demonstrated that the SQUIDs in this system show minimal hysteresis after three de-Gaussing cycles. Once tuning was complete, the ADR ramped up to 303~mK and remained there for launch. At 6~minutes before launch, the LHe pumping valve was closed. The instrument was then in launch configuration and passed pre-launch checks. 

\begin{table} [htb]
	\begin{centering}
	\begin{tabular}{l|c|l|l|l}
		%\hline
		\bf{Flight time} & \bf{Event} & \bf{He bath [K]} & \bf{FEA [mK]} & \bf{Magnet current [mA]}\\
		\hline
		%T - 10:30~hr & Report on station & - \\
		%T - 10:00~hr & V-Phi tests & - \\
		T - 8:55~hr &  LHe transfer & 4.314
		$\pm$ 0.002 & 3278 $\pm$ 55 & 0 $\pm$ 5 \\
		%\hline
		%T - 5:10~hr & \multicolumn{4}{c}{\textit{Payload power off for arming}}\\
		T - 5:10~hr & Power off for arming & 1.898 $\pm$ 0.001 & 1510 $\pm$ 9 & 0 $\pm$ 5  \\
		%\hline
		%T - 3:40~hr & ADR ramp up & - & 1653 $\pm$ 6 & - \\
		%T - 3:05~hr & Full field & - & 2360 $\pm$ 40 & 9414 $\pm$ 6 \\
		T - 3:40~hr & ADR ramp up to full field & 1.986 $\pm$ 0.001 & 2442 - 1573 $\pm$ 50 & 9397.3 $\pm$ 5 \\
		%T - 1:38~hr & ADR ramp down to 75~mK & \hl{1.956 $\pm$ 0.001} & \hl{75.000 $\pm$ 0.011} & \hl{264 $\pm$ 1} \\	
		%\hline
		T - 1:35~hr & SQUID tuning & 1.956 $\pm$ 0.001 & 74.972 $\pm$ 0.006 & 264 - 210 $\pm$ 5  \\
		& & & 75.62 $\pm$ 0.01 & \\
		T - 18~min & ADR ramp up to 300~mK & 1.96 - 2.05 $\pm$ 0.001 & 324 $\pm$ 21 mK & 73 - 112 $\pm$ 3\\
		& & & 317 $\pm$ 33 mK \\
		%T - 6~min & Close BTS & 1.961 $\pm$ 0.001 & - & - \\
		%\hline
		T = 0 & Ignition & 2.054 $\pm$ 0.001~K & 324 $\pm$ 21 mK & 1.191 $\pm$ 0.005 A \\
		& & & 317 $\pm$ 33 mK \\
		\hline
	\end{tabular}
	\caption{The pre-flight events controlling the cryostat and ADR prepared the instrument for flight. }
	\label{Countdown}
	\end{centering}
\end{table}
%\bigskip
%
%\subsubsection{Commanding}
%\label{CountdownCommanding}
%
%All commanding was nominal (Table \ref{Countdown-ADR-commands}, Figure~\ref{countdown-adrc-commands}). The ADR commands are a combination of the Ramp Up, Ramp Down, Fast Ramp, and GRT Scale commands. To regulate, both the Ramp Up and Ramp Down commands are actuated. To hold, neither the Ramp Up nor Ramp Down commands are actuated. 
%
%The ADR started the countdown in the Ramp Down state, with the Fast Ramp low and the GRT Scale high. Ramp Down is the default state; if left in the Hold state, the magnet current slowly rises. The GRT Scale is designed to change from high to low at 350~mK, and it was therefore kept high until the ADR was ramped down. It then was kept low for the remainder of the countdown. 
%
%The ADR was taken out of Ramp Down and set to Hold for the duration of the Horizontal and Vertical Checks to minimize confusion during testing (i.e., both Ramp Up and Ramp Down are low). It was then  powered off during arming. After arming and the launcher raise, power was restored to the payload, and the ADR magnet cycle began: it was ramped up to full field, the cold stage was allowed to thermalize, then the heat switch was opened and it was ramped down to regulate at 75~mK. To optimize this process, the ADR was ramped down to 85~mK and then set to regulate to 75~mK. After taking a magnet current measurement, the ADR was ramped up to 300~mK and held there until tuning.
%
%\begin{table} [h]
%	\begin{centering}
%	\begin{tabular}{llll}
%		\hline
%		\bf{Time} & \bf{Event} & \bf{ADR State} & \bf{GRT Scale}\\
%		\hline
%		T - 10~hr & Start of countdown & Ramp Down & High\\
%		T - 5:57~hr & Horizontal checks & Hold & High\\
%		\textit{T - 4:40~hr} & \textit{Power off for arming} & - & - \\
%		\hline
%		T - 3:10~hr & ADR Ramp Up & Ramp Up; Fast Ramp & High\\
%		\it{T - 3:00~hr} & \it{Move T-time to midnight} & - & - \\
%		T - 2:20~hr & ADR Ramp Down to 85~mK & Ramp Down; Fast Ramp & Low\\
%		T - 2:10~hr & ADR Regulate to 75~mK & Regulate & Low\\
%		T - 2:08~hr & ADR Ramp Up to 300~mK & Ramp Up; Fast Ramp & Low\\
%		T - 2:00~hr & ADR Hold at 300~mK & Hold & Low\\
%		T - 1:57~hr & Vertical checks & Hold & Low\\
%		T - 1:38~hr & ADR Ramp Down to 85~mK & Ramp Down; Fast Ramp & Low\\
%		T - 1:36~hr & ADR Regulate at 75~mK & Regulate & Low \\
%		T - 1:35~hr & Tuning & All commands & Low\\
%		\hline
%		T - 18~min & ADR Ramp Up to 300~mK & Ramp Up; Fast Ramp & Low \\
%		T - 16~min & ADR Hold at 300~mK & Hold & Low\\
%		T = 0 & Ignition & Hold & Low \\
%		\hline
%	\end{tabular}
%	\caption{ADR Command countdown}
%	\label{Countdown-ADR-commands}
%	\end{centering}
%\end{table}
%
%\bigskip
%
%\begin{figure} [htp]
%	\begin{center}
%		\vcenteredhbox{\includegraphics[width=\textwidth]{figs/countdown_adr-commands.png}}
%	\end{center}
%	\caption{ADR commands (from top): Ramp Up, Ramp Down, Fast Ramp, and GRT Scale.} 
%	\label{countdown-adrc-commands}
%\end{figure}
%
%\bigskip
%\bigskip
%
%\begin{table} [h]
%	\begin{centering}
%	\begin{tabular}{lll}
%		\hline
%		\bf{Time} & \bf{Event} & \bf{GaAs [K]} \\
%		\hline
%		T - 7:35~hr & Start pumpdown & 4.325 $\pm$ 0.003 \\
%		T - 4:40~hr & Power off for arming & 1.9 $\pm$ 0.1\\
%		T - 3:40~hr & Launcher raise & 2.060 maximum\\
%		\hline
%		\it{T - 3:00~hr} & \it{Move T-time to midnight} & - \\
%		\hline
%		T - 2:25~hr & Open heat switch & 1.986 $\pm$ 0.001\\
%		T - 2:10~hr & ADR Regulate to 75~mK & 1.956 $\pm$ 0.001 \\
%		T - 1:35~hr & Tuning & 1.961 $\pm$ 0.001 \\
%		\hline
%		T - 6~min & Close BTS & 1.961 $\pm$ 0.001 \\
%		T = 0 & Ignition & 2.052 \\
%		\hline
%	\end{tabular}
%	\caption{Cryostat Performance [distributions are from 1~min intervals]}
%	\end{centering}
%	\label{Countdown-ADR}
%\end{table}
%
%\newpage
\begin{figure} [htp]
	\begin{center}
			\includegraphics[width=\textwidth]{figs/countdown_combined.png}
			%\includegraphics[width=\textwidth]{figs/countdown_thermals_%full.png}
			%\includegraphics[width=\textwidth]{figs/countdown_inset.png}
		%\includegraphics[width=\textwidth]{figs/countdown_thermals_horizontal.png}
		\end{center}
	\caption{Thermal behavior during the countdown, including the LHe bath pumpdown and the ADR magnet cycle; inset details the tuning and flight operations. From top: LHe bath temperature, detector array temperature, and ADR magnet current. The instrument was powered off during arming, and the data during this period is not valid. Noise picked up by ground operations prior to the deGaussing cycles appears as occasional points that significantly deviate from the general trend of the signal. These points are sparse enough that they do not noticeably contaminate the readout data.}
	\label{countdown-thermals}
\end{figure}

\bigskip

%\begin{figure} [htp]
%	\begin{center}
%		\includegraphics[width=\textwidth]{figs/hotcount_thermals_edited.png}
%	\end{center}
%	\caption{Thermal behavior from tuning until impact: He bath t%	\label{hotcount-thermals}
%\end{figure}
%
%\newpage
%\subsubsection{Electrical Performance}
%\label{Preflight Rails}
%
%Electrical performance was nominal throughout the launch countdown across both flight and GSE hardware. 
%
%The ADRC performance was healthy during the countdown. The data rate remained a constant 82.2 $\pm$ 0.2~kbit/s; the apparent data drop during tuning is due to the hardware setup. Time measurements remained consistent and showed no data loss (Figures \ref{countdown-health}, \ref{countdown-time}). Temperature sensors, located on 4 components in the ADRC, measured the temperature of these components (Table \ref{AD590Table}, Figure~\ref{countdown-ad590s}). One was not operating; the highest observed temperature on any sensor was 28.2$^\circ$C. Each voltage rail through the Magnet Power Supply was monitored and all rails were nominal throughout the countdown (Table \ref{AD590Table}, Figures \ref{countdown-35s}, \ref{countdown-15s}, \ref{countdown-magnet}). Electrical health in flight is described in \S \ref{Electrical Health}. 
%
%\bigskip
%
%\begin{figure} [htp]
%	\begin{center}
%		\vcenteredhbox{\includegraphics[width=\textwidth]{figs/countdown_health.png}}
%	\end{center}
%	\caption{System health: data rate} 
%	\label{countdown-health}
%\end{figure}
%
%\bigskip
%
%\begin{figure} [htp]
%	\begin{center}
%		\vcenteredhbox{\includegraphics[width=\textwidth]{figs/countdown_time.png}}
%	\end{center}
%	\caption{System health: time} 
%	\label{countdown-time}
%\end{figure}
%
%\bigskip
%
%\begin{table} [h]
%	\begin{centering}
%	\begin{tabular}{lllll}
%		\hline
%		\bf{} & \bf{AD590 (1)} & \bf{AD590 (2)} & \bf{AD590 (3)} & \bf{AD590 (4)}\\
%		\hline
%		\textbf{Location} & - & - & - & - \\
%		\textbf{He transfer [$^\circ$C]} & 6.5 & - & 4.5 & 6.4\\
%		\textbf{Launch temp [$^\circ$C]} & 23.8 & - & 27.4 & 28.2\\
%		\hline
%	\end{tabular}
%	\caption{Electronics component temperatures in-flight}
%	\label{AD590Table}
%	\end{centering}
%\end{table}
%
%\bigskip
%
%\begin{figure} [htp]
%	\begin{center}
%		\vcenteredhbox{\includegraphics[width=\textwidth]{figs/countdown-ad590s.png}}
%	\end{center}
%	\caption{AD590s} 
%	\label{countdown-ad590s}
%\end{figure}
%
%\newpage
%
%Power during the countdown came from the power busses in the TM section. These busses were powered externally from lab supplies through the umbi for most of the countdown. They were powered by the flight batteries starting at the Hot Count at T-10~min. 
%
%\bigskip
%
%\bigskip
%
%\begin{figure} [htp]
%	\begin{center}
%		\vcenteredhbox{\includegraphics[width=\textwidth]{figs/countdown_vmon-35.png}}
%	\end{center}
%	\caption{Voltage monitors: 3.2V (top), 5V (bottom)} 
%	\label{countdown-35s}
%\end{figure}
%
%\bigskip
%
%\begin{figure} [htp]
%	\begin{center}
%		\vcenteredhbox{\includegraphics[width=\textwidth]{figs/countdown_vmon-15.png}}
%	\end{center}
%	\caption{Voltage monitors: $\pm$15V} 
%	\label{countdown-15s}
%\end{figure}
%
%\bigskip
%
%\begin{figure} [htp]
%	\begin{center}
%		\vcenteredhbox{\includegraphics[width=\textwidth]{figs/coundown_magnet.png}}
%	\end{center}
%	\caption{Voltage rails and magnet power (from top): 28V rail Reg in, Mag Supply, Mag CTL, Mag $\times$ 200N} 
%	\label{countdown-magnet}
%\end{figure}

==> sections/flight-resolution.tex <==
% !TEX root = ../instrument_paper_revB.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Energy Resolution}
\label{sec:EnergyResolution}

% \dcom{Northwestern discussed the pixel array map vs readout arrangement. Thought readout made more sense because there wasn't a science result and it shows correlations better. Maybe want to include blank pixel map in the detector section for archival.}

The X-rays observed in flight were all consistent - in energy and event rate - with the on-board calibration source (\S \ref{sec:Calibration Source}). This is expected with the ACS failure; several astronomical X-ray sources passed through the instrument's field of view during the science observation as labeled in Figure~\ref{fig:RADec_time} but none were bright enough to accumulate a detectable number of counts. The average count rate was $0.7$~counts/pixel/s, corresponding to a K-K$\alpha$ rate of 0.23~$\pm$~0.06~counts/pixel/s and matching the pre-flight rate observed from the calibration source. Despite not having any time on target during flight, x-rays from the on-board calibration source were used to characterize the detector response. %One of the more important performance specifications is energy resolution because that is what sets Micro-X apart from other x-ray experiments (\S \ref{sec:Intro}).

\subsubsection{Payload Configurations \& Data}

It is useful to compare the detector resolution to pre-flight performance to understand the impact that a space environment has on TES and SQUID performance. Data taken with the experiment in three different configurations will be compared: laboratory data, integration data, and flight data.

\paragraph{Laboratory Data} The laboratory data shown was taken in a laboratory at Northwestern University in April 2018, a few months before flight. During that run only one science chain was able to run at a time, thus data was collected from half of the pixels per data set.
%Data was collected from half of the pixels at a time due to hardware available limiting data taking to one science chain at a time. 
The readout electronics boxes were physically separated from each other on different carts and tabletops. The TES bias was set to 7500 \hl{units?} for all columns, which is slightly higher than the bias that was used for flight.

\paragraph{Integration Data} The integration data shown was taken in a laboratory at WSMR two weeks prior to flight on July 9\&10, 2018. This data was taken with the rocket built up in flight configuration. Mechanically, the cryostat was bolted to the optics and electronics sections and encased in the rocket skin. The electronics stacks were placed near each other at the forward end of the cryostat and both science chains were run simultaneously, which means that two power supplies were on, two master clocks were running, and twice as many cables were installed. In keeping with standard sounding rocket convention, electrical connectors were encased in plastic backshells and potted. Metal sheaths were placed around the power cables, and nylon sheaths were used for all other cables. All cables were tightly bound and laced for routing inside the skin. The TES bias was set to 6500 \hl{units?}, which is slightly lower in the transition than the laboratory data but was the same value used for flight.
% Integration resolution trigger: 4096 ms auto, 50 mV edge
% Integration NEP trigger: 50 mV edge, noise = 0

\paragraph{Flight Data} The flight data was taken %with the rocket fully built up and flying 
in space on July 22, 2018. The data was collected on all pixels via the two science chains, stored in on-board flash memory, and uploaded after the rocket was recovered. The flash data was then played back and broken up into individual traces of 4096 digital sample points, 512 of which are pre-trigger for calculating and subtracting the baseline level. The gain was set so that pulses register as negative voltages and they were triggered using a derivative-based edge trigger. % that was set at -0.05~V/ms, which is generally faster than most transient backgrounds.
A level trigger was used to collect noise traces that did not exceed the derivative edge trigger threshold.% the edge trigger and were less than 1000~mV.
The TES bias was set to 6500 \hl{units?} for all columns.

\subsubsection{Data Cuts \& Initial Analysis}

Analysis was performed using IGOR Pro from WaveMetrics. When a triggered data file is loaded in IGOR the triggering information is not conveyed, so the first cut on the data is a loose threshold cut above the root mean square of the baseline noise to identify traces containing a pulse. The second cut is to set a time window in the trace where a pulse is expected to trigger based on the pre-trigger, risetime, and falltime of the pulse. Any trace whose maximum amplitude is above the noise threshold cut and outside the time window cut is rejected; most commonly these are traces with more than one trace from the calibration source or pileup events.

The next step is to prepare the inputs for the Optimal Filtering (OF) algorithm, which involves making a template of the average pulse and average noise for each pixel. The average pulse is calculated by selecting events in the K-K$\alpha$ calibration line using a box cut in a plot of raw pulse height versus time. A quality cut is also applied to the average pulse by rejecting any events that were selected that have a large chi-squared as compared to the average; roughly 10\% of the selected traces are removed via this cut. In a well-behaved dataset such as the laboratory data, all of the noise traces can be averaged before applying a similar chi-squared cut as used for the average pulse. However, due to the unexpected unlocking of the SQUIDs during flight, a box cut in a plot of baseline versus baseline slope was used to select noise from times when the detectors were live. The average pulse and noise are then 
%passed to the OF that fits the templates to each pulse in frequency space and calculates a rough energy calibration using the pulse height and the known energy of the template pulse.
used to construct the OF and noise-equivalent power (NEP) in frequency space. The NEP is used to approximate the baseline energy resolution of the detector given the signal and noise, presented in the next section (\S\ref{sec:NEP}). The OF is convolved in the time domain with each signal and noise triggered trace. The maximum of this convolution is used as the uncalibrated energy estimate for that pulse or noise trace. A rough energy calibration using the pulse height and the known energy of the template pulse is used to scale the data. The data is then further calibrated as detailed in \S~\ref{sec:specResolution}. 

\subsubsection{Baseline Energy Resolution Estimates from NEP}
\label{sec:NEP}

\acom{Citation for optimal filter needed? Noah's thesis? What about NEP? } The noise-equivalent power (NEP) is a measure of the system noise at each frequency compared to a reference response from a known energy input to the system. The energy input is usually photons from an X-ray calibration source. The integral of the inverse of the NEP$^2$ provides an estimate of the intrinsic baseline energy resolution. This estimate assumes a linear energy scale from zero to the calibration line energy. The K-K$\alpha$ line is the strongest in the Micro-X calibration source (\S \ref{sec:Calibration Source}) and is used throughout the data processing pipeline. The baseline resolution estimate from the integral of the NEP will be referred to as ``NEP" in the following sections, has units of eV, and its accuracy has been validated against Gaussian fits of the calibrated noise spectrum in Figure~\ref{fig:resolution_method_comparison}.

Figure~\ref{fig:NEP_readout} shows NEP maps of individual pixels for the three datasets and indicates that detector performance significantly depends on the mechanical and electrical configuration of the instrument. The laboratory data demonstrates the best performance with the lowest and most consistent NEPs. The NEPs get notably worse after the instrument is integrated into flight configuration. The specific mechanism of this degradation is not understood, but integrating the instrument brought the mechanical and electrical components into much closer proximity. Running both telemetry master clocks simultaneously (one for each independent readout chain of the SQUID MUX) introduces a beat frequency between 60--100~Hz that impacted energy resolution. %is seen in the baseline of the detector readouts in Figure~\ref{flightpulses}. 
Synchronizing the master clocks was demonstrated in post-flight testing to remove this beating, and this clock synchronization will be implemented for future flights (\S \ref{sec:Reflight}).

\begin{figure} 
	\centering
% 	\includegraphics[width=0.3\textwidth]{figs/combined_lab_data_NEP_readout.png}
% 	\includegraphics[width=0.3\textwidth]{figs/combined_integration_data_NEP_readout.png}
% 	\includegraphics[width=0.3\textwidth]{figs/combined_flight_data_NEP_readout.png}
	\includegraphics[width=\textwidth]{figs/NEP_readout_all3.png}
	\caption{Plot of NEPs from the laboratory configuration approximately three months prior to flight (left), the integration configuration roughly two weeks prior to flight (center), and during flight (right). The dark gray pixels are known non-operational pixels, and the light gray pixels had insufficient statistics for calculating the NEP.}
	\label{fig:NEP_readout}
\end{figure}

Table~\ref{tab:NEP_ranges} shows the number of pixels within given ranges of NEPs. Although most of the pixels unlocked at some time during flight (Figure~\ref{fig:Pulse_times}), there were only fifteen pixels that did not have enough statistics to calculate an NEP. Disregarding those pixels, most of which are on readout column XA, the flight NEPs are consistent with the integration data. This means the flight environment did not significantly degrade the detector resolution. This table also highlights the resolution degradation as almost half of the pixels with NEPs between 5--15~eV in the laboratory configuration give resolutions $>$15~eV after integration. The cumulative degradation can also be seen in Figure~\ref{fig:cumulative_neps} that shows the resolution distribution of the full array.

\begin{table}
\begin{center}
\begin{tabular}{ |c|c|c|c| } 
    \hline
    NEP Range [eV] & Laboratory & Integration & Flight \\ 
    \hline
    0-5   & 2 & 2 & 0 \\ 
    5-15  & 113 & 59 & 60 \\ 
    15-25 & 1 & 29 & 27 \\ 
    25+   & 0 & 27 & 14 \\ 
    Dead/Unlocked & 12 & 11 & 27 \\ 
    \hline
\end{tabular}
\caption{Binned NEPs from laboratory, integration, and flight data. The consistency between integration and flight performance can be seen, as well as the degraded resolution compared to laboratory operation.}
\label{tab:NEP_ranges}
\end{center}
\end{table}

\begin{figure} 
	\centering
% 	\includegraphics[width=0.9\textwidth]{figs/paper_cumulative_nep_fraction.png}
% 	\includegraphics[width=0.9\textwidth]{figs/paper_hr_cumulative_nep_fraction.png}
	\includegraphics[width=0.45\textwidth]{figs/comparing_NEP_hists.png}
    \includegraphics[width=0.45\textwidth]{figs/CDF_NEP.png}
	\caption{Plots comparing NEPs from the laboratory, integration, and flight datasets. The left plot is a histogram and the right plot is a cumulative distribution function. \acom{Left stronger as pixel-pixel scatter plots}}
	\label{fig:cumulative_neps}
\end{figure}

% These pixels have a demonstrated energy resolution of 4.5~eV in a stable, non-MUXing laboratory environment \hl{cite}.
% In the laboratory configuration, 106 of the pixels in the array achieved an NEP better than 10~eV at 3.3~keV.
% At launch, 116 of the 128 TES pixels were operational.
% Detector performance was strongly impacted both by the instrument configuration (\S \ref{sec:configuration}) and external magnetic fields (\S \ref{Flight Magetic Field}). Modifications have been implemented to mitigate these effects as discussed in \S \ref{sec:Reflight}.
% The behavior observed in flight has been confirmed with subsequent testing on the ground, and post-flight noise testing also demonstrated that the ADR system was not a discernible source of noise. 

There are two primary inputs for the NEP calculation: signal and noise. Therefore, it's reasonable to ask which is responsible for the degraded NEPs after the rocket has been integrated.
It is most natural to look at pulse shapes in the time domain. Figure~\ref{fig:example_pulses} shows the average of K-K$\alpha$ current pulses for a few example pixels. The plot on the left shows a pixel with different pulse shapes and sizes between the three datasets, yet the NEP was consistently low (under 10~eV). The plot on the right shows a pixel with a relatively consistent pulse size between datasets; in fact, the average pulses from integration and flight are nearly identical. However, the NEP for this pixel shows the resolution degraded 3x once the payload was integrated. While this is only a small selection of pixels, both examples prove that the pulse shape is not the dominant factor in the resolution degradation across the array.

%  Sample pulses from the science observation are shown in Figure~\ref{flightpulses}.
%  \begin{figure}
% 	\includegraphics[width=0.4\textwidth,keepaspectratio]{figs/YD_pulses.eps}
% 	\caption{K-K$\alpha$ pulses from the on-board calibration source during the flight science observation. An artificial offset is applied for clarity. Oscillations in the baseline are due to beating between the encoder clocks. \hl{Being remade}}
% 	\label{flightpulses} 
% \end{figure}

\begin{figure}
    % \includegraphics[width=0.45\textwidth]{figs/Example_pulse_goodpix.png}
    % \includegraphics[width=0.45\textwidth]{figs/Example_pulse_badpix.png}
    % \includegraphics[width=0.45\textwidth]{figs/Example_pulse_goodpix_YD09.png}
    \includegraphics[width=0.45\textwidth]{figs/Example_pulse_goodpix_YD10.png}
	\includegraphics[width=0.45\textwidth]{figs/Example_pulse_badpix_YD00.png}
	\caption{Average K-K$\alpha$ pulses for two pixels. The pixel on the left has a similar NEP across datasets despite different pulse shapes and sizes, while the pixel on the right has consistent pulse shapes yet severe NEP degradation.}
	\label{fig:example_pulses} 
\end{figure}

Comparing average noise between pixels is easiest when looking at plots of the power spectral density (PSD) to see which, if any, frequencies are being picked up. The PSD is calculated from the average of fast fourier transforms (FFTs) of noise traces.% and average pulses on a pixel. 
Since the NEP is effectively a signal-to-noise ratio, having a larger area between the average pulse and noise PSD will result in better resolving power. PSDs for the same pixels as Figure~\ref{fig:example_pulses} are shown in Figure~\ref{fig:example_PSDs}. The data that has NEPs $>$15~eV clearly shows an elevated noise level at frequencies below 1~kHz. The conclusion from this is that decreasing the proximity between electronics components during integration increased the amount of noise coupling into the system, resulting in degraded NEPs across the array.\tcom{Antonia should chime in here about what our conclusions should be.}

\begin{figure}
% 	\includegraphics[width=0.45\textwidth]{figs/Example_noise_goodpix.png}
% 	\includegraphics[width=0.45\textwidth]{figs/Example_noise_badpix.png}
% 	\includegraphics[width=0.45\textwidth]{figs/Example_noise_goodpix_YD09.png}
	\includegraphics[width=0.45\textwidth]{figs/Example_noise_goodpix_YD10.png}
	\includegraphics[width=0.45\textwidth]{figs/Example_noise_badpix_YD00.png}
	\caption{Average PSDs for two pixels, one with a low NEP before and after integration (left) and one with increased noise pick up after integration (right). The lines at the top of the plots are FFTs of the same average pulses shown in Figure~\ref{fig:example_pulses}. \acom{How many pules in average pulse/noise? Add an example of white noise degradation in IT to flight.}}
	\label{fig:example_PSDs} 
\end{figure}


\subsubsection{Spectral Resolution}
\label{sec:specResolution}

Beyond the resolution approximation based on the NEP, the data was further processed to make calibrated energy spectra that were fit to measure the actual energy resolution of the detectors. The processing done to refine the data falls into four steps:

\begin{enumerate}
    \item \textbf{Baseline correction:} performs a linear fit of the K-K$\alpha$ calibration line to correct for any steady changes in the baseline such as temperature drifts. This step is not complex enough to correct for the payload tumbling in the Earth's magnetic field.
    \item \textbf{Lagphase correction:} corrects for error in determining the pulse height due to digitization of the signal.
    \item \textbf{Drift correction:} corrects for variation in the gain by fitting a spline to the K-K$\alpha$ calibration line. In theory, this could correct for the changing external magnetic field, but the limited statistics on each pixel made it difficult to accurately fit the erratic behavior.
    \item \textbf{Gain calibration:} fits each calibration line (Cl-K$\alpha$, Cl-K$\beta$, K-K$\alpha$, K-K$\beta$, and Mn-K$\alpha$) to get the observed energy and then calibrates the gain as a function of expected energy with an n-degree polynomial, where n is the number of calibration lines fit minus one.
\end{enumerate}

The calibrated energy spectrum from 0--6~keV for side Y is shown in Figure~\ref{fig:full_spectrum}. If there had not been an ACS failure, this would be an important plot for identifying peaks in the science region of interest. As it is, the Cl-K$\alpha$ and K-K$\alpha$ peaks from the calibration source (\S \ref{sec:Calibration Source}) are clearly evident, as well as the K$\beta$ associated with each decay. A hint of the Mn-K$\alpha$ peak can even be seen just below 6~keV. The spectrum for a single pixel is included to compare the relative peak heights. 

\begin{figure}
	\includegraphics[width=0.9\textwidth]{figs/CalibratedSpectrum_allSideY_YD09.png}
    \caption{Calibrated energy spectrum of pulses from side Y during the science observation window. The blue line is all pixels on side Y co-added except for the known dead pixels (dark gray pixels in Fig.\ref{fig:NEP_readout}. The red line is a single pixel, the same one shown in Fig.~\ref{fig:spectral_fits}. \acom{Let's make co-added only; remove legend/title (single pixel covering full spectrum/misleading since we have such different exposures.)} \acom{Are the low energy events (not visible here, but there are some!) astrophysical??}}
	\label{fig:full_spectrum} 
\end{figure}

With the calibrated energy spectrum, a Gaussian fit of the noise events around 0~eV gives the baseline resolution of the detectors. Figure~\ref{fig:resolution_method_comparison} shows a histogram of the baseline resolutions and the NEP resolutions from flight. %The flight environment was not as stable as running the experiment in a laboratory on the ground. 
The data processing improves the resolution by $\sim$10\%, likely due to the difference between the linear energy calibration of the NEP and the polynomial energy calibration of the flight data.\tcom{we should check this}

\begin{figure}
	\includegraphics[width=0.6\textwidth]{figs/resolution_comparison1.png}
	\caption{Comparison of resolution methods using flight data. The NEP accurately estimates the baseline resolution to within approximately 10\%. \acom{Add what pixels are cut off from this and from reported paper numbers}}
	\label{fig:resolution_method_comparison} 
\end{figure}

Figure~\ref{fig:spectral_fits} shows a number of examples of individual fits to calibrated energy spectra, where the full width at half maximum (FWHM) of the fit gives the detector resolution for a given x-ray photon energy. Notice the lower statistics in the flight data due to the short flight time and loss of livetime, hence those fits have worse chi-squares and bigger uncertainty on the measured resolution. The drift in baseline due to tumbling during flight and the low statistics makes correcting for energy scale drifts versus time very challenging. The comparison of the NEP estimates to the baseline resolution (the top row in Figure~\ref{fig:spectral_fits}) gives us confidence that with higher statistics and a stable platform during flight, energy resolutions closer to the integration data will be achieved in flight.
\acom{Add co-added spectrum, both zoomed in and zoomed out. Okay to select only some pixels for it, but need to explicitly say who was included. }

% \begin{figure}
%     \includegraphics[width=0.8\textwidth, keepaspectratio]{figs/FlightSpectrum_BW.eps}
% 	\caption{Co-added spectrum of the K-K$\alpha$ line from the on-board calibration source across the 6 best pixels in flight. \hl{Remaking}}
%     \label{flightspec}
% \end{figure}

\begin{figure}
	\includegraphics[width=0.3\textwidth]{figs/lab_0eV_YD09.png}
	\includegraphics[width=0.3\textwidth]{figs/integrated_0eV_YD09.png}
	\includegraphics[width=0.3\textwidth]{figs/flight_0eV_YD09.png}
	\includegraphics[width=0.3\textwidth]{figs/lab_Cla_YD09.png}
	\includegraphics[width=0.3\textwidth]{figs/integrated_Cla_YD09.png}
	\includegraphics[width=0.3\textwidth]{figs/flight_Cla_YD09.png}
	\includegraphics[width=0.3\textwidth]{figs/lab_Ka_YD09.png}
	\includegraphics[width=0.3\textwidth]{figs/integrated_Ka_YD09.png}
	\includegraphics[width=0.3\textwidth]{figs/flight_Ka_YD09.png}
	\caption{Spectral line fits for a single example pixel (YD09) that was one of the best - low resolution with sufficient statistics - for all three datasets. The left column is laboratory data, the center column is integration data, and the right column is flight data. The top row is a fit to the noise events centered on 0~eV, the middle row is a fit to the Cl-K$\alpha$ line, and the bottom row is a fit to the K-K$\alpha$ line. The residual between the data and the fit is shown at the bottom of each plot.\tcom{we'll remake this plot with larger text and take out the file names which are not interesting to readers.} \acom{Dan following up on: if we are already so much broader at 0 keV from system noise, why such a big degradation to higher energies?}}
	\label{fig:spectral_fits} 
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% With the exception of the external magnetic field effects, exacerbated by the ACS failure, no change to the noise spectrum or pulse shape was observed between ground and flight. \acom{This was the statement in SPIE paper, but I think we've now shown it's not correct}
% Within the flight data, no change was observed to the noise spectrum or pulse shape between those periods when the array was open or closed to space (i.e., the shutter door and aperture valve open or closed).
% The following sections describe the impact of external magnetic fields on the SQUIDS (\S\ref{sec:SQUID_magnetic_susceptibility}) and TESs (\S\ref{sec:TES_magnetic_susceptibility}), and the resolution and noise response of the instrument on the ground (\S\ref{sec:preflight_performance}) and in flight (\S\ref{sec:flight_resolution_performance}). 


% The system was then integrated for flight (the "integrated configuration"), at which point 39~pixels maintained an NEP better than 10~eV, and 76 pixels maintained an NEP better than 20~eV. The best pixel in this configuration achieved an NEP of 4.4~eV, as seen in Figure~\ref{fig:integration_NEP_readout}.


% \begin{figure}
% %\begin{wrapfigure}{l}{0.49\textwidth}
% 		\begin{center}
% 			\includegraphics[width=0.45\textwidth, keepaspectratio]{figs/lab_nep.PNG}
% 		\includegraphics[width=0.45\textwidth, keepaspectratio]{figs/temp_preflight_nep.PNG}
% 			\caption{\label{preflight_neps} NEP of each pixel in the laboratory configuration (left) and integrated before flight (right). \hl{Remaking}}
% 		\end{center}
% 	\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\section{Impact of ACS Pointing Failure}
%\label{Flight Magetic Field}
%
%\begin{enumerate}
%    \item Measurements and plots for mag field
%    \item Josh \& Joe plots on SQUID unlocks due to mag field
%    \item Josh on detector response to mag field (pulse height and decay times)
%    \item Detector Performance Section
%\end{enumerate}
%
%
%\subsection{SQUID Performance}
%\label{sec:SQUID Performance}
%
%The magnetic field encountered in flight from the Earth's field is measured by the three-axis magnetometer in the telemetry section, and its response is confirmed through its agreement with the projected Earth's field. The projected field inputs the rocket location and orientation into the International Geomagnetic Reference Field (IGRF) model \hl{cite} to derive the local magnetic field. The projected and measured magnetic fields are shown in Figure~\ref{Magnetometers}, in excellent agreement with each other until the parachute descent. 
%Trajectory information from the ground radar and pointing data from the ACS were used with The International Geomagnetic Reference Field (IGRF) model managed by the International Association of Geomagnetism and Aeronomy (IAGA) to calculate the Earth's magnetic field in the rocket's frame. This was used to check the calibration of the magnetometers.

%Specifically, time, longitude, latitude, and altitude data was used in the IGRF to get the Earth's magnetic field, given in North/South, East/West, and Up/Down. The pointing information in right ascension and declination was used to convert this into the rocket rest frame. The calculated Earth's magnetic field for the Z-direction and for the total field is showed by dashed lines in \ref{Magnetometers}  
%
%
%\begin{figure} [htp]
%	\begin{center}
		%\includegraphics[width=0.7\textwidth]{figs/mag_temp.png}
%		\includegraphics[width=0.8\textwidth]{figs/MagnetometersPlaceHolder.png}
%	\end{center}
%	\caption{\hl{This will be magnetometer data plot for the absolute field from X, Y, Z, total, snout. dB/dt for the same.How do we want to distinguish the calculated field? }}
%	\label{Magnetometers}
%\end{figure}
%
%Many of the SQUIDs ``lost lock" in flight, meaning that they deviated far enough from their operational settings that their feedback loops were unstable, and their associated TES could not be read out. Analysis of the rocket ascent and science observation indicate that the unlocking is likely due to a susceptibility to external magnetic fields at the SQ2 stage. While the rocket always spins during powered flight, the pointing failure led the rocket to continue spinning during the science observation, which would not happen in a normal flight.  Figure~\ref{fig:flight_unlocked} shows that the unlocking is not instantaneous across the entire array, but does broadly track by TDM column, consistent with the SQ2 driving the effect. The resulting fractional livetime for each pixel is shown in Figure~\ref{livetime}. This behavior appeared for the first time in flight; it was not observed in laboratory operations or in ground operations in the days before launch. 
%	
% \begin{figure}[hbt]
% 	\begin{center}
% 		\includegraphics[width=0.8\textwidth, keepaspectratio]{figs/temp_flight_unlocking.PNG}
% 		\caption{Placeholder for image about magnetic field and losing lock.  \acom{AH: Renee will make new image; pixel naming should match between images.}	\label{fig:flight_unlocked}}
% 	\end{center}
% \end{figure}
%
% \begin{wrapfigure}{r}{0.4\textwidth}
% 	\includegraphics[width=0.4\textwidth,keepaspectratio]{figs/livetime_plot.eps}
% 	\caption{\label{livetime} Distribution of fractional livetime across the array, where 1.0 corresponds to reading out during the entire science obervation (as was the case for 15\% of the array). The corresponding deadtime is due to the SQUID readouts losing lock. \acom{Redo- Northwestern}}
% \end{wrapfigure}
%
%\begin{figure}
%    \centering
%    \begin{subfigure}[t]{0.48\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figs/LockedPlot_sideX_fullflight.png}
%        \caption{Side X Locked Plot}
%        \label{fig:SideX_LockedPlot}
%    \end{subfigure}
%    \hfill
%    \begin{subfigure}[t]{0.48\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figs/LockedPlot_sideY_fullflight.png}
%        \caption{Side Y Locked Plot}
%        \label{fig:SideY_LockedPlot}
%    \end{subfigure}
%    \caption{Plots indicating times during flight when SQUIDs were able to maintain lock and read out the corresponding TES.}
%    \label{fig:LockedPlots}
%\end{figure}
%
%\begin{figure}
%    \centering
%    \begin{subfigure}[t]{0.48\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figs/Liv%etime_SideX_observation.png}
%        \caption{Side X Livetime}
%        \label{fig:SideX_LivetimePlot}
%    \end{subfigure}
%    \hfill
%    \begin{subfigure}[t]{0.48\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figs/Liv%etime_SideY_observation.png}
%        \caption{Side Y Livetime}
%        \label{fig:SideY_LivetimePlot}
%    \end{subfigure}
%    \caption{Plots of the fractional livetimes when %the SQUIDs were locked during the science observation window.}
%    \label{fig:LivetimePlots}
%\end{figure}
%
%
%At launch, the first motor stage ignited, and the rocket spun up to \hl{x}~rotations/s. It then burned out, and the second motor stage ignited, spinning the rocket up to \hl{4.5}~rotations/s. The de-spin then slowed the rocket spin to \hl{x}~rotations/s. During powered flight, the ADR was holding at 321~mK, and the TES were therefore normal. The recorded data is thus indicative only of the behavior of the SQUIDs. The untriggered feedback signal during this period strongly correlates with the Earth's magnetic field in the direction of the holes in the Nb can for the science chain cables, as shown in Figure~\ref{fig:ascent}. The external field is believed to couple the strongest to the SQ2 stage, which is consistent with the SQ2 stage having an effective area that is nearly two orders of magnitude larger than the SQ1 stage (\S\ref{sec:FEA}). The MUX06a SQ2s used in the first flight are known to be particularly susceptible to external magnetic fields~\citep{Stiehl:2011}. \hl{Statement on new FEA not being as susceptible.} 
%
%\begin{figure} [htp]
%	\begin{center}
%		\includegraphics[width=0.7\textwidth]{figs/ascent_correlation.png}
%	\end{center}
%	\caption{The untriggered SQUID feedback signal tracks the magnetic field in the direction of the cable holes in the Nb magnetic shield during the rocket ascent. The TES are normal in this period, so the correlation is due to the response of the SQUIDs to external magnetic fields. \hl{Remake}}
%	\label{fig:ascent}
%\end{figure}
%
%During the science observation, the rocket spun with an average roll rate of 1.6$^\circ$/s, and a maximum rate of 4.7$^\circ$/s. The ADR was in tight temperature control, and the TES were in the transition during this period. The baseline of the SQUID response continued to track the external magnetic field in the direction of the holes in the Nb can holes during throughout the science observation. \hl{Insert more of Josh's analysis.} 
%
%During the parachute descent, the magnetic field is unstable and unpredictable. In this portion of the flight, the projected magnetic field from the Earth's field deviates from the observed field in the magnetometer, and the SQUID response no longer tracks the Earth's field in the direction of the Nb can holes. This unstable magnetic field is a known phenomenon in sounding rocket flights. \hl{Josh:  Have we verified this is true?} Its exact origin is unknown, but it is hypothesized that the hot rocket skin breeds a plasma around the rocket as it descends, creating an unpredictable and unmodeled magnetic field environment. This unpredictable environment is empirically confirmed by both the magnetometer and SQUID responses. 
%
%During the observation period, the rocket tumbles at a maximum of 4.7 degrees per second and an average of 1.6 degrees per second. \hl{( Do we want to add the max roll rate?)}. The maximum roll rate during observation was 1.2 degrees per second. \hl{do we want the theta, phi, theta rate, and phi rate graphs}

%While the the total magnetic field varies from 0.42 to 0.48 Gauss \hl{this is from the calculated magnetic field}, the magnetic field in the(x,y,z)- direction varies from \hl{(X,Y,Z) to (X,Y,Z), respectively}. \hl{As the magnetic field at the FEA is the most important measurement, the magnetic field data was rotated to additionally monitor the field in the direction of the ``snouts" in the Nb shield (do we want to show the snout direction graph?)} (\S \ref{sec:Shielding}), shown in Figure~\ref{Magnetometers}.

%The payload spun throughout the flight due to the pointing failure. This spinning is not part of a normal flight trajectory, and it caused the magnetic field to change directions beyond what the instrument is engineered to withstand. This changing magnetic field is the leading hypothesis for the source of the SQUIDs unlocking in flight. As described further in \S \ref{sec:Flight Detectors}, it has been demonstrated in subsequent laboratory testing that a changing external field of this magnitude consistently unlocks the SQUIDs. This is not anticipated to be a concern for future flights with proper pointing. Nevertheless, modifications have been made to the instrument to mitigate this effect on future flights in case the pointing failure was not the sole source of unlocking (\S \ref{sec:Reflight}). 
%
%To study the impact of external fields on the flight system, post-flight testing with Helmholtz coils reproduced spinning in the Earth's field. These tests did cause the SQUIDs to unlock. \acom{Soften/elaborate on this.} The hysteretic response of the SQUIDs to changing magnetic fields precludes a precise reproduction of the flight response, \hl{but the SQUIDs that unlocked in flight were repeatedly found to be the most susceptible to unlocking in Helmholtz coil testing.} \acom{Include a plot to back up statement.} \hl{However, a predictive correspondence between magnetic field and SQ2 unlocking has not been demonstrated. Multiple mitigation strategies, described in} \S \ref{sec:Reflight}, \hl{have been implemented for future flights. }
%
%\bigskip 
%
%\begin{table} [h]
%	\begin{centering}
%	\begin{tabular}{llll}
%		\hline
%		\bf{Time} & \bf{Event} & \bf{Thrust field (X) [V]} & \bf{Total field [V]}\\
%		\hline
%		T = 0 & Launch & 6.5 & 25.2\\
%		T + 111.3 - 430.8~s & Science observation & 14.1 - 33.8 & 29.7 - 50.2 \\
%		T + 596 - 780.0~s & Calibration data & 8.2 - 40.3 & 21.7 - 38.7\\
%		\hline
%	\end{tabular}
%	\caption{Magnetometer flight events}
%	\end{centering}
%\end{table}
%
%\bigskip
%
%\begin{figure} [htp]
%	\begin{center}
%		\includegraphics[width=\textwidth]{figs/total_magnetic_field.png}
%	\end{center}
%	\caption{Magnetometer data (from top): Z-direction, X-direction, Y-direction, total \com{Update with Renee's plot}}
%	\label{Magnetometers}
%\end{figure}	\caption{On-board flight electronics. The dashed line marks the interface between the science instrument and NSROC telemetry. \acom{clearly aspect ratio is artificial... rethink layout and what to emphasize visually. Vibrometers. Add other telemetry sensors? (Magnetometers/accelerometers)} }
%
%\subsection{Detector Mag Field Response}
%
%\textbf{Josh's TES response to mag field.}
%\textbf{item 3 above}
%

%%%%%%%%%%%%%%%%%%%%

% Detector performance significantly depends on the mechanical and electrical configuration of the instrument. These pixels have a demonstrated energy resolution of 4.5~eV in a stable, non-MUXing laboratory environment \hl{cite}. The initial configuration (the "laboratory configuration") took data with only one science chain instrumented, and with the electronics boxes on the benchtop. In this configuration, 106 of the pixels in the array achieved an NEP better than 10~eV at 3.3~keV, as seen in Figure~\ref{preflight_neps} (left). The system was then integrated for flight (the "integrated configuration"), at which point 39~pixels maintained an NEP better than 10~eV, and 76 pixels maintained an NEP better than 20~eV. The best pixel in this configuration achieved an NEP of 4.4~eV, as seen in Figure~\ref{preflight_neps} (right). The specific mechanism of this degradation is not understood, but integrating the instrument changed both the mechanical and electrical configurations. Mechanically, the cryostat was bolted to the optics and electronics sections. The electronics stacks, which run physically separated in the laboratory configuration, were placed near each other (and near the forward end of the cryostat) in their flight configuration. In keeping with standard sounding rocket convention, electrical connectors were encased in plastic backshells and potted, rather than using metal backshells. Metal sheaths were placed around the power cables, and nylon sheaths were used for all other cables. Electrically, both science chains were run simultaneously, which was not the case in the laboratory configuration, in which only half of the array was read out. Reading out the full array means that two power supplies were on, two master clocks were running, and twice as many cables were installed. Running both clocks simultaneously introduces a beat frequency that is seen in the baseline of the detector readouts in Figure~\ref{flightpulses}. Synchronizing the master clocks was demonstrated in post-flight testing to remove this beating, and this clock synchronization will be implemented for future flights (\S \ref{sec:Reflight}). Post-flight noise testing also demonstrated that the ADR system was not a discernible source of noise. 

% Flight detector performance is consistent with the integrated configuration. Exposing the detectors to space did not change their performance. Detector response is indistinguishable between the science observation (when the detectors are exposed to space) and directly after the aperture valve and shutter door were closed in preparation for re-entry, as shown in \hl{(Figure~x)}. The noise spectrum and pulse shape is indistinguishable between the two configurations, demonstrating that the detectors are not seeing any impact from the telemetry antennae or other sources of radio noise. It also demonstrates that any infrared or optical light that may be present, although unexpected, is blocked by the filters. Thus an optimization of performance on the ground is predicted to indicate future flight performance. \hl{Megan: not on Hitomi, where NEP looked the same but resolution did not}

% Nineteen pixels, including one entire column, stayed locked over the entire science observation, and the total equivalent science observation exposure across all pixels was \hl{50~s}. To demonstrate the capability of this instrument in future flights, the six pixels with the best energy resolution were co-added for the spectrum shown in Figure~\ref{flightspec}. The spectrum includes \hl{568} events and returns a Full-Width Half-Maximum (FWHM) energy resolution of \hl{12.98}~eV at \hl{3.3}~keV (Figure~\ref{flightspec}). \hl{These same six pixels all achieved NEPs of X in laboratory testing, and X in integrated pre-flight testing.}  \acom{Elaborate on how this is representative of future flights.} 

%The 19 pixels that stayed locked over the entire science observation were used for the flight performance analysis. Their gain drifted by roughly 60~eV over the course of the science observation, which is significantly larger than their projected energy resolution. Their gain drifted to $\sim$2\% of their pulse heights. 

	

==> sections/mission_overview.tex <==
% !TEX root = ../instrument_paper_revB.tex
\section{Mission Overview}
\label{sec: Mission Overview}

\subsection{Astrophysics Program}

The Micro-X science program focuses on observations of SNRs (\S \ref{SNRs}) and indirect detection of galactic dark matter (\S \ref{DM Science}). The primary target for SNR observations is the Bright Eastern Knot (BEK) of the Puppis A SNR, and the secondary target is Cassiopeia A. The primary dark matter target is a quiet X-ray region just off the galactic plane, and the secondary target is the Galactic Center. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Supernova Remnants}
\label{SNRs}
\input{sections/SNR_science}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Dark Matter}
\label{DM Science}
\input{sections/dark_matter}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{TES Microcalorimeters}
\label{sec:TES_intro}

Microcalorimeters are cryogenic X-ray detectors that provide excellent energy resolution in the keV regime. They consist of an X-ray absorber, a thermometer, and a weak thermal link to connect the absorber with a heat sink, as shown in Figure~\ref{fig:TES} (left). When an X-ray of energy $E$ is incident on the pixel, the temperature of the absorber rises by $\Delta T \approx \frac{E}{C}$, where  $C$ is the heat capacity of the absorber. As the deposited heat dissipates into the heat sink, the absorber cools back down with the time constant %proportional to the natural time constant,
$\tau \propto \tau_o = \frac{C}{G}$, where $G$ is the thermal conductivity of the weak thermal link. This creates the characteristic ``pulse" observed by the thermometer, shown in Figure~\ref{fig:TES} (center). Additional information on microcalorimeters can be found in~\cite{McCammon2005}. 

\begin{figure}[htb]
	\centering
	\includegraphics[width=\textwidth]{figs/RvsT.pdf}
	\caption{When an X-ray is incident on a TES microcalorimeter (left), the temperature of the absorber rises, then returns to its base temperature as heat dissipates through the weak thermal link. The size and shape of the pulse (center) observed by the TES thermometer depend on the energy of the X-ray (E), the heat capacity of the absorber (C) and the thermal conductivity of the thermal link (G). The resistance of the TES sharply changes with the temperature in the absorber (right). The size of the response depends on where the TES is biased in its superconducting transition and the slope of the transition ($\alpha$).}
	\label{fig:TES}
	\vspace{-5pt}
\end{figure}

Micro-X uses Transition-Edge Sensors (TES) as its microcalorimeter thermometers. A TES is a superconducting film operating at a stable, cryogenic temperature that places it between its superconducting and normal resistance ranges. In this transition regime, shown in Figure~\ref{fig:TES} (right), the small temperature change from an absorbed X-ray produces a large change in the TES resistance, and the energy of the X-ray can thus be reconstructed to high precision. The slope of the TES transition is given by the dimensionless parameter $\alpha = \frac{T}{R} \frac{dR}{dT}$. Operationally, the cold bath is kept colder than the TES transition temperature, and a voltage bias is applied to the TES to warm it into the transition through Joule heating. The power deposited through Joule heating is inversely proportional to the resistance of the TES, 
%($P \propto \frac{1}{R(T)}$), 
%expressed as P = $\frac{V^2}{R(T)}$, 
so as the temperature (and therefore resistance) increases, the applied power decreases, and the TES cools back down. This electrothermal feedback mechanism speeds up the return of the TES to its stable position in the transition after an X-ray event. The TES response has a resulting decay time of $\tau \simeq \tau_0 /(1 + \frac{\alpha P_o}{T_o G})$, where $P_o$ and $T_o$ are the quiescent power and temperature, respectively. TES microcalorimeters have achieved energy resolutions down to 1.6~$\pm$~0.1~eV  for 6.89~keV X-rays in a stable laboratory environment~\citep{Smith:2012, Minuissi:2018}. The Micro-X readout scheme is specifically described in \S~\ref{sec:FEA}. 
%TESs are conventionally read out with SQUIDs, which serve as amplifiers. Micro-X uses a TDM SQUID readout scheme that is specifically described in \S \ref{sec:FEA}.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Sounding Rockets}

Sounding rockets are suborbital missions that provide approximately five minutes of observation above the atmosphere~\citep{SRHB}. X-rays in the Micro-X signal bandpass are attenuated by the atmosphere, so they can only be observed above 160~km altitude. Sounding rocket payloads can be recovered after flight with the ability to re-fly, making them a particularly good testbed for new technologies, as with Micro-X. Specialized engineering is required to successfully operate sensitive detectors, like microcalorimeters, in the vibrationally violent and time-constrained conditions of a sounding rocket flight. 

%The first Micro-X flight launched from the White Sands Missile Range (WSMR) in New Mexico on July 22, 2018.
The payload, shown in Figure~\ref{fig:Payload}, includes the science instrument (\S \ref{sec:Instrument}) and several standard payload systems that are supplied by the NASA Sounding Rocket Operations Contract (NSROC)~\cite{SRHB}. These systems include an Ogive Recovery System Assembly (ORSA) to control the descent, a celestial attitude control system (ACS) for pointing, a S-19 boost guidance system for trajectory control, and three telemetry links for data transmission. The telemetry antennae include one 5~W and two 10~W (minimum) transmitters. The 5~W transmitter has a carrier frequency of 2279.5~MHz, with the 10~W transmitters at 2235.5~MHz and 2382.5~MHz. %The payload is designed to provide a $\ge$300~second observation above an altitude of 160~km. The ACS was provided to point the telescope at the Cas A science target at (RA, Dec) = (350.85$^\circ$, 58.815$^\circ$). Details on the NSROC components can be found in the Sounding Rocket Handbook~\cite{SRHB}. 
The rocket is a two-stage Terrier MK70 Black Brant IX MK4. 

\begin{figure}[htb]
	\begin{center}
		%\includegraphics[width=\textwidth]{figs/payload.png}
		\includegraphics[width=\textwidth]{figs/Mirco-X-Integrated-pic.png}
	\end{center}
	\caption{The Micro-X payload includes the science instrument and standard rocket systems for flight operations, including data transmission (telemetry), trajectory control (S-19), pointing (ACS), and a parachute for the descent (ORSA). The rocket motors are not shown. }
	\label{fig:Payload}
\end{figure} 
